Parallel Programming Models for Heterogeneous Many-Cores : A Survey

Heterogeneous many-cores are now an integral part of modern computing systems ranging from embedding systems to supercomputers. While heterogeneous many-core design offers the potential for energy-efficient high-performance, such potential can only be unlocked if the application programs are suitably parallel and can be made to match the underlying heterogeneous platform. In this article, we provide a comprehensive survey for parallel programming models for heterogeneous many-core architectures and review the compiling techniques of improving programmability and portability. We examine various software optimization techniques for minimizing the communicating overhead between heterogeneous computing devices. We provide a road map for a wide variety of different research areas. We conclude with a discussion on open issues in the area and potential research directions. This article provides both an accessible introduction to the fast-moving area of heterogeneous programming and a detailed bibliography of its main achievements.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=svjour3

SAMPLES = \
	main.tex 


PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.tex   $(PACKAGE).cls *.tex *.bib
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	#open *.pdf
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM) *.log *.aux *.bbl *.blg \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi ${PDF}

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> lst/source_out.tex <==
__kernel void A(__global char* a, short b, int c) {
  const int d = get_global_id(0);
  a[d] = b;
}

==> pp-models - Copy/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=svjour3

SAMPLES = \
	main.tex 


PDF = ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.tex   $(PACKAGE).cls *.tex *.bib
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	#open *.pdf
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM) *.log *.aux *.bbl *.blg \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi ${PDF}

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf $(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE) 

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> pp-models - Copy/bridge.tex <==
%\section{The Bridge between High-level, Low-level and Domain Models}
%\section{Source-to-Source Compiling Techniques for Improving Programmability and Portability} \label{sec:bridge}
%\section{Compiling Techniques for Better Programmability and Portability} \label{sec:bridge}
\section{Compiling Techniques for Improved Programmability and Portability} \label{sec:bridge}
Translating code in one programming model to another enables code reuse and reduce the learning curve of a new computing language.
Ultimately, code translation can improve programmability, portability, and performance.
In this section, we review the code translation techniques between parallel programming models on heterogeneous many-core architectures.
%There are three methodologies in translating between computing frameworks: (1) Add an abstract level library among
%frameworks; (2) Translate to a common intermediate representation (IR) and compile the IR during run-time; or (3) Translate
%a source code that uses a particular framework to a modified source code that uses a different framework.

%to support multiple compute devices

% serial code to CUDA
%\cparagraph{C-to-CUDA}
\vspace{-2mm}
\subsection{C-to-CUDA}
%Graphics Processing Units (GPUs) offer tremendous computational power.
CUDA provides a multi-threaded parallel programming model,
facilitating high performance implementations of general-purpose computations on GPUs.
However, manual development of high-performance CUDA code still requires a large amount of effort from programmers.
Programmers have to explicitly manage the memory hierarchy and multi-level parallel view.
%make manual development of high-performance CUDA code rather complicated.
Hence the automatic transformation of sequential input programs into parallel CUDA programs is of significant interest.
%A number of parallelizing source-to-source compilers have recently been developed to
%ease programming of multi-core and many-core processors.

%Recent advances in multi-core and many-core processors requires programmers to
%exploit an increasing amount of parallelism from their applications.
%Data parallel languages such as CUDA and OpenCL make it possible to take advantage of such processors,
%but still require a large amount of effort from programmers.

Baskaran \etal describe an automatic code transformation system that generates parallel CUDA code from input sequential C code,
for affine programs~\cite{DBLP:conf/cc/BaskaranRS10}.
Using publicly available tools that have made polyhedral compiler optimization practically effective,
the authors develop a C-to-CUDA transformation system that generates two-level parallel CUDA code
that is optimized for efficient data access.
%The performance of automatically generated code is compared with manually optimized CUDA code for a number of benchmarks.
The performance of the automatically generated CUDA code is close to hand-optimized versions
and considerably better than their performance on multi-core CPUs.
Building on Baskaran's experience, Reservoir Labs developed its own compiler based on R-Stream~\cite{DBLP:conf/asplos/LeungVMBWBL10},
which introduces a more advanced algorithm to exploit the memory hierarchy.
%R-Stream appears to be using a more
%advanced scheduling algorithm than PPCG and automatically determines the required
%tile sizes, whereas PPCG currently expects these to be provided by the user. However,
%the paper glosses over many of the details, and no source code is available to inspect.


\cparagraph{PPCG} Verdoolaege \etal address the compilation of a sequential program for parallel execution
on a modern GPU~\cite{DBLP:journals/taco/VerdoolaegeJCGTC13}.
They present a source-to-source compiler (\texttt{PPCG}),
which singles out for its ability to accelerate computations from any static control loop nest,
generating multiple CUDA kernels when necessary.
The authors introduce a multilevel tiling strategy and
a code generation scheme for the parallelization and
locality optimization of imperfectly nested loops,
managing memory and exposing concurrency according to the constraints of modern GPUs.
%They evaluate our algorithms and tool on the entire PolyBench suite~\cite{DBLP:journals/taco/VerdoolaegeJCGTC13}.

\cparagraph{Bones}
Nugteren \etal evaluate a number of C-to-CUDA transformation tools targeting GPUs,
%, focused in particular on C-to-CUDA transformations targeting GPUs.
%We compare these tools both qualitatively and quantitatively to each other
and identify their strengths and weaknesses~\cite{DBLP:conf/asplos/NugterenC12}.
Then they address the weaknesses by presenting a new classification of algorithms.
This classification is used in a source-to-source compiler (\texttt{Bones}) based on the algorithmic skeletons technique.
The compiler generates target code based on skeletons of parallel structures,
which can be seen as parameterisable library implementations for a set of algorithm classes.
%We furthermore demonstrate that the presented
This compiler still requires some modifications to the original sequential source code, but
can generate readable code for further fine-tuning.
%and delivers superior performance compared to other tools for a set of 8 image processing kernels.

\cparagraph{PIPS} Non-polyhedral tools have also seen major developments. PIPS
is an open-source initiative developed by the HPC Project to unify
efforts concerning compilers for parallel architectures~\cite{pips_url, DBLP:conf/lcpc/AminiCIK11}.
It supports the automatic integrated compilation
of applications for heterogeneous architectures including GPUs.
The compiler
%is not based on the polyhedral model, but
uses abstract interpretation for array regions based on polyhedra,
%which also involves polyhedra;
which allows PIPS to perform powerful interprocedural analysis on the input code.

% C to OpenMP/OpenACC
%\subsection{C-to-Directive}
\cparagraph{DawnCC}
%Directive-based programming models, such as OpenACC and OpenMP, allow developers to
%convert a sequential program into a parallel one with minimum human intervention.
%However,
Mendonca \etal argue that inserting pragmas into production code is a difficult and error-prone task,
often requiring familiarity with the target program~\cite{DBLP:journals/taco/MendoncaGAPAP17, DBLP:conf/cgo/MishraKC19}.
This difficulty restricts developers from annotating code
that they have not written themselves.
Therefore, they provide a suite of compiler-based methods and a tool, \texttt{DawnCC}, to mitigate the issue.
%Such techniques
The tool relies on symbolic range analysis
%, a well-known static technique,
to achieve two purposes: populate source code with data transfer primitives and
to disambiguate pointers that could hinder automatic parallelization due to aliasing.
%We have materialized our ideas into a tool, DawnCC, which can be used stand-alone or through an online interface.
%To demonstrate its effectiveness, we show how DawnCC can annotate the programs available in PolyBench
%without any intervention from users.
%Such annotations lead to speedups of over 100x in an Nvidia architecture and over 50x in an ARM architecture.

% Code translation between CUDA and OpenCL
\vspace{-2mm}
\subsection{CUDA-to-OpenCL}
Restricted to NVIDIA GPUs, CUDA has the largest code base and high-performance libraries.
On the other hand, OpenCL is an open standard supported on a large number of mainstream devices.
With the great interest in OpenCL comes a challenge:
manufacturers have a large investment in CUDA codes and yet would
like to take advantage of wider deployment opportunities afforded by OpenCL.
%Given the similarities between CUDA and OpenCL,
%manually porting a CUDA application to OpenCL is typically straightforward, but tedious and error-prone.
Therefore, an automated tool for CUDA-to-OpenCL translation is required.

%With a choice in programming environments comes the need to choose.
%CUDA has the largest installed base and many time-saving libraries for important functions such as FFT.
%However, it is only supported on NVIDIA hardware.
%OpenCL, on the other hand,
%is an open standard that is supported on a variety of mainstream devices: NVIDIA GPUs, AMD GPUs,
%and x86/x86–64 CPUs from Intel and AMD.
%Support is also available for some system-on-chip (SoC) devices, including the ARM Cortex-A9 CPU and the PowerVR SGX GPU.
%Additionally, Intel intends to support OpenCL on their Many Integrated Cores (MIC) architecture,
%and Altera already has a program to develop an OpenCL environment for their FPGAs.
%Due to the greater functional portability provided by OpenCL, many are choosing OpenCL as their programming environment of choice.

%With the great interest in OpenCL comes a challenge: organizations have a large investment in CUDA codes and yet would
%like to take advantage of wider deployment opportunities afforded by OpenCL.
%Thus, there needs to be a translator from CUDA to OpenCL that
%not only allows compilation in the new environment but also yields maintainable source code such
%that development can continue directly in OpenCL.

%To this end, we created CU2CL, an automatic CUDA-to-OpenCL
%source-to-source translator that also preserves the comments and formatting in the original source code.

%Heterogeneous systems are widening their user-base, and heterogeneous computing is becoming popular in supercomputing.
%Among others, OpenCL and CUDA are the most popular programming models for heterogeneous systems.
%Although OpenCL inherited many features from CUDA and they have almost the same platform model,
%they are not compatible with each other.

\cparagraph{SnuCL-Tr}
Kim \etal present similarities and differences between CUDA and OpenCL, and develop an automatic translation framework
between them~\cite{DBLP:conf/sc/KimDJJL15}.
%In particular, they describe features that make it difficult to translate from one to the other and provide a solution.
%This translator
\texttt{SnuCL-Tr}
can achieve comparable performance between the original and target applications in both directions.
Given that each programming model has a large user-base and code-base,
this translator is useful to extend the code-base for each programming model and
unifies the efforts to develop applications.
% for heterogeneous systems.

\cparagraph{CU2CL}
Gardner \etal summarize the challenges of translating CUDA code to its OpenCL equivalence~\cite{DBLP:journals/pc/GardnerSFM13}.
%Over the past decade, accelerator-based supercomputers have grown from 0\% to 42\% performance share on the TOP500.
%Ideally, GPU-accelerated code on such systems should be "write once, run anywhere,"
%regardless of the GPU device (or for that matter, any parallel device, e.g., CPU or FPGA).
%In practice, however, portability can be significantly more limited due to the sheer volume of code implemented
%in non-portable languages. For example, the tremendous success of CUDA,
%as evidenced by the vast cornucopia of CUDA-accelerated applications,
%makes it infeasible to manually rewrite all these applications to achieve portability.
%Consequently, we achieve portability by using our
They develop an automated CUDA-to-OpenCL source-to-source translator (\texttt{CU2CL}),
%To demonstrate the state of the practice, they
to automatically translate three medium-to-large,
CUDA-optimized codes to OpenCL, thus enabling the codes to run on other GPU-accelerated systems~\cite{DBLP:conf/hpcasia/SathreGF19, DBLP:conf/icpads/MartinezGF11}.
%These automatically translated codes deliver performance portability, including as much as three-fold performance improvement, on a GPU device not supported by CUDA.
%Closer to CU2CL's goal,
\texttt{Swan} is tool used to ease the transition between OpenCL and CUDA~\cite{DBLP:journals/cphysics/HarveyF11}.
%However, Swan is not actually a source-to-source translator like CU2CL;
%instead
Different from CU2CL, Swan provides a higher-level library that abstracts both CUDA and OpenCL,
such that an application makes calls to Swan and Swan
%takes care of the details in mapping to CUDA or OpenCL.
takes care of mapping the calls to CUDA or OpenCL.
%The Swan API is limited, as it currentlyonly abstracts a few features in common between CUDA and OpenCL.
%On the other hand, it
%Swan provides a simple Perl scriptthat can automatically translate kernel codes,
%by performing a regular expression-based search and replace operation on the source.
%Much of the work, however, is left up to the developer to port his or her application (especially host code)
%and its kernels to use Swan's libraries.

\cparagraph{NMT}
Kim \etal present source-to-source translation between CUDA to OpenCL using neural machine translation (\texttt{NMT}).
%The contribution of the work is that it develops techniques to generate training inputs.
To generate a training dataset, they extract CUDA API usages from CUDA examples and write corresponding OpenCL API usages.
With a pair of API usages acquired, they construct API usage trees that help users find unseen usages
from new samples and easily add them to a training input~\cite{DBLP:conf/cgo/KimK19}.
%The initial results show that NMT can translate many applications from benchmarks
%such as CUDA SDK, polybench-gpu, and Rodinia.
%Furthermore, we show that translated kernel code from CUDA applications can be run in the OpenCL FPGA framework,
%which implies a new direction of HLS.

% OpenCL to renderscript
\cparagraph{O2render}
%More than half-a-billion Android devices are world's most impactful real-time,
%interactive multimedia systems that are open-sourced.
%Google introduced Renderscript language and runtime in Android releases starting in 2011.
%Renderscript delivers performance and portability without losing usability.
%However, it is difficult to reuse software written in existing compute languages such as OpenCL.
%Thus,
With a similar goal, Yang \etal introduces \texttt{O2render}, an OpenCL-to-Renderscript
translator that enables the porting of an OpenCL application to
a Renderscript application~\cite{DBLP:conf/estimedia/YangWL12}.
O2render automatically translates
OpenCL kernels to a Renderscript kernel.
%, or can create a
%skeleton of Renderscript script from an OpenCL kernel to
%enable developers to port OpenCL kernel more rapidly.
%develop the O2render system to enable OpenCL programs on Android devices~\cite{DBLP:conf/estimedia/YangWL12}.
%We analyze fundamental differences between OpenCL and Renderscript,
%and present our design of a translator between them using low-level virtual machine (LLVM).
%We extend LLVMs frontend, Clang, and show that we achieve about the same performance
%in Renderscript with minimal translation overhead.



% Directive-based lang to CUDA
\vspace{-2mm}
\subsection{Directive-to-CUDA/OpenCL}

%GPGPUs have recently emerged as powerful vehicles for general-purpose high-performance computing.
%Although a new ComputeUnified Device Architecture (CUDA) programming model from NVIDIA
%offers improved programmability for general computing,programming GPGPUs is still complex and error-prone.

%Graphics Processing Units (GPUs) have become a competitive accelerator for applications outside the graphics domain,
%mainly driven by the improvements in GPU programmability.
%Although the Compute Unified Device Architecture (CUDA) is a simple C-like interface for programming NVIDIA GPUs,
%porting applications to CUDA remains a challenge to average programmers.
%In particular, CUDA places on the programmer the burden of packaging GPU code in separate functions,
%of explicitly managing data transfer between the host and GPU memories,
%and of manually optimizing the utilization of the GPU memory.
%Practical experience shows that the programmer needs to make significant code changes,
%often tedious and error-prone, before getting an optimized program.
Translating OpenMP-like codes into CUDA/OpenCL codes will not only reuse the large OpenMP code base,
but also lower their programming barrier.

\cparagraph{OpenMP-to-CUDA}
Lee and Eigenmann present a framework for automatic source-to-source
translation of standard OpenMP applications into CUDA applications~\cite{DBLP:conf/ppopp/LeeME09}.
%The goal of this translation
This translator aims to further improve programmability and make existing OpenMP applications
amenable to execution on GPGPUs.
Later, they propose a new programming interface, \texttt{OpenMPC},
which builds on OpenMP to provide an abstraction of CUDA and
offers high-level controls of the involved parameters and optimizations~\cite{DBLP:conf/sc/LeeE10}.

\cparagraph{OpenMP-to-OpenCL}
Kim \etal propose a framework that translates OpenMP 4.0 accelerator directives to OpenCL~\cite{DBLP:conf/sc/KimLPL16}.
They leverage a run-time optimization to automatically eliminates unnecessary data transfers
between the host and the accelerator.
%The authors have identified several key transformation techniques, which enable efficient
%GPU global memory access, to achieve high performance.
%Experimental results from two important kernels (JACOBI and SPMUL)
%and two NAS OpenMP Parallel Benchmarks (EP and CG) show
%that the described translator and compile-time optimizations work
%well on both regular and irregular applications, leading to performance improvements of up
%to 50X over the unoptimized translation
%(up to 328X over serial on a CPU).

% One directive to another
\cparagraph{OpenMP-to-LEO}
%Intel MIC (Many Integrated Core) is the first x86-based coprocessor architecture aimed at accelerating multi-core HPC applications.
%In the most common usage model, parallel code sections are offloaded to the MIC coprocessor using LEO (Language Extensions for Offload).
%The developer is responsible for identifying and specifying offloadable code regions,
Managing data transfers between the CPU and XeonPhi and optimizing applications for performance
requires some amount of effort and experimentation.
%In~\cite{DBLP:conf/ics/RaviYBC12},
Ravi \etal present \texttt{Apricot}, an optimizing compiler and productivity tool for Intel XeonPhi
%x86-compatible many-core coprocessors
% (such as Intel MIC)
that minimizes developer effort by automatically inserting LEO clauses~\cite{DBLP:conf/ics/RaviYBC12}.
 %for parallelizable code regions,
%(ii) selectively offloading some of the code regions to the coprocessor at runtime
%based on a cost model that we have developed,
%(iii) applying a set ofoptimizations for minimizing the data communication overhead and improving overall performance.
%Apricot
This optimizing compiler aims to assist programmers in porting existing multi-core applications and
writing new ones to take full advantage of the many-core accelerator,
while maximizing overall performance.
%Experiments with SpecOMP and NAS Parallel benchmarks show that
%Apricot can successfully transform OpenMP applications to run on the MIC coprocessor with good performance gains.

%CUDA and its underlying GPUs offer multiple memory types
%with different bandwidth, latency, and access restrictions to allow programmers
%to conserve memory bandwidth while increasing the overall performance of their
%applications. Currently, CUDA programmers are responsible for explicitly allocating space
%and managing data movement among the different memories to
%conserve memory bandwidth. Furthermore, additional hardware mechanisms at
%the memory interface can enhance the main memory access efficiency if the access patterns
%follow memory coalescing rules.
\cparagraph{CUDA-lite}
CUDA programmers shoulder the responsibility of managing the code to produce the desirable access patterns.
Experiences show that such responsibility presents a major burden on the programmer, and
this task can be better performed by automated tools.
Ueng \etal present \texttt{CUDA-lite}, an enhancement to CUDA, as one such tool~\cite{DBLP:conf/lcpc/UengLBH08}.
This tool leverages programmers' knowledge via annotations to perform transformations and
show preliminary results that indicate auto-generated code can have performance comparable to hand-crafted codes.

\cparagraph{hiCUDA}
Han \etal have designed \texttt{hiCUDA}~\cite{DBLP:journals/tpds/HanA11, DBLP:conf/asplos/HanA09},
a high-level directive-based language for CUDA programming.
%It allows programmers to perform these tedious tasks in a simpler manner and directly to the sequential code,
%aiming to speed up the porting process.
%In this paper, we describe the hiCUDA directives as well as the design and implementation of a prototype compiler
%that translates a hiCUDA program to a CUDA program.
They develop a prototype compiler to facilitate the translation of a hiCUDA program to a CUDA program.
The compiler is able to support real-world applications that span multiple procedures and use dynamically allocated arrays.
%Experiments using nine CUDA benchmarks show that the simplicity hiCUDA provides comes at no expense to performance.

%\cparagraph{Mint}
%Unat \etal present Mint, a programming model that enables the non-expert to enjoy the performance benefits of
%hand coded CUDA without becoming entangled in the details~\cite{DBLP:conf/ics/UnatCB11}.
%Mint targets stencil methods, which are an important class of scientific applications.
%We have implemented t
%The Mint programming model has been implemented with a source-to-source translator that
%generates optimized CUDA C from traditional C source.
%The translator relies on annotations to guide translation at a high level.
%The set of pragmas is small, and the model is compact and simple.
%Yet, Mint is able to deliver performance competitive with painstakingly hand-optimized CUDA.
%We show that, for a set of widely used stencil kernels, Mint realized 80\% of the performance
%obtained from aggressively optimized CUDA on the 200 series NVIDIA GPUs.
%Our optimizations target three dimensional kernels,
%which present a daunting array of optimizations.

\cparagraph{CUDA-CHiLL} The CHiLL developers extended their compiler to generate GPU code
with \texttt{CUDA-CHiLL}~\cite{DBLP:conf/lcpc/RudyKHCC10},
%;they introduced CUDA-CHiLL~\cite{DBLP:conf/lcpc/RudyKHCC10},
which does not perform an automatic
parallelization and mapping to CUDA but instead offers high-level constructs that
allow a user or search engine to perform such a transformation.


% Converting CUDA/OpenCL for Multi-core CPUs
\subsection{Adapting CUDA/OpenCL to Multi-core CPUs}
\cparagraph{MCUDA} is a source-to-source translator
that translates CUDA to multi-threaded CPU code~\cite{DBLP:conf/lcpc/StrattonSH08}.
This translator is built on Cetus~\cite{DBLP:journals/ijpp/BaeMLALDEM13},
a source-to-source translator framework for C and other C-based languages.

\cparagraph{CUDA-x86} by PGI allows developers using CUDA to compile and optimize their CUDA applications
to run on x86-based multi-core architectures~\cite{cudax64_url}.
%workstations, servers and clusters with or without an NVIDIA GPU accelerator.
\texttt{CUDA-x86} includes full support for NVIDIA's CUDA C/C++ language for GPUs.
%so that programmers can recompile CUDA code for execution on an x86 architecture.
When running on x86-based systems without a GPU,
%PGI CUDA C applications
CUDA applications can use multiple cores and the streaming SIMD capabilities of Intel and AMD CPUs for parallel execution.
%With PGI CUDA C compilers, CUDA developers now can have a common code path for both NVIDIA GPU and x86 platform.

\cparagraph{Ocelot}~\cite{DBLP:conf/IEEEpact/DiamosKYC10} is primarily a PTX-to-LLVM translator and
run-time system that can decide whether to run the PTX on a GPU device or on a CPU with just-in-time (JIT) compilation.
\texttt{Ocelot} is similar to \texttt{MCUDA} in that it allows for CUDA kernels to be run on CPUs,
but it takes the approach of performing translations on lower-level bytecodes.
%In today's compilers,
%This is a typical approach to take,
%converting a higher-level language to some intermediate representation and then compiling it to the target architecture.


==> pp-models - Copy/conclusions.tex <==
\section{Conclusions}
 This article has introduced programming models for heterogeneous many-core architectures. Power, energy and thermal limits have
forced the hardware industry to introduce heterogeneous many-cores built around specialized processors. However, developers are struggling
to manage the complexity of heterogeneous many-core hardware. A crisis is looming as these systems become pervasive. As such, how to enable
developers to write and optimize programs for the emerging heterogeneous many-core architectures has generated a large amount of academic
interest and papers. While it is impossible to provide a definitive cataloger of all research, we have tried to provide a comprehensive and
accessible survey of the main research areas and future directions. As we have discussed in the article, this is a trustworthy and exciting
direction for systems researchers.


==> pp-models - Copy/domain.tex <==
%\subsubsection{Domain-Specific Parallel Programming Models}
\subsubsection{Domain-Specific Programming Models}
%When using heterogeneous multi-core platforms to solve problems in specific fields, 
%researchers will also use domain specific attributes
%Domain specific language (DSL) takes into account both program performance and programmability, 
%rather than directly using the native heterogeneous programming model. 
To achieve an even better performance and programmability, the domain-specific programming models are preferred on heterogeneous many-cores.

%In~\cite{ops_tr}, 
Mudalige \etal propose a high-level programming framework, \texttt{OPS},  
for multi-block structural grid applications~\cite{ops_tr}. 
The frontend of \texttt{OPS} leverages a common set of APIs for users, 
and the backend generates highly optimized device code for target platforms. 
%Experiments show that the OPS code can produce performance matching the original code. 
The \texttt{OP2} framework is built upon \texttt{OPS}.
%framework continues the basic idea of op2 framework. 
The difference is that \texttt{OPS} is suitable for dealing with multi-block structured grids, 
while \texttt{OP2} is targeted for unstructured grid applications~\cite{DBLP:journals/sigmetrics/GilesMSMK11}.
%[50].
\texttt{AMGCL} is a header-only C++ library for solving large sparse linear systems with algebraic multigrid (AMG) method~\cite{Demidov2019}. 
%AMG is one of the most effective iterative methods for solution of equation systems arising, for example, 
%from discretizing PDEs on unstructured grids [BrMH85], [Stue99], [TrOS01]. 
%The method can be used as a black-box solver for various computational problems, 
%since it does not require any information about the underlying geometry. 
%AMG is often used not as a standalone solver but as a preconditioner 
%within an iterative solver (e.g. Conjugate Gradients, BiCGStab, or GMRES).
This library has a minimal dependency, and provides both shared-memory and distributed memory versions of the algorithms. 
%The AMG hierarchy is constructed on a CPU and then is transferred into one of the provided backends. 
It allows for transparent acceleration of the solution phase with OpenCL, CUDA, or OpenMP~\cite{denis_demidov_2018_1244532}. 
%Users may provide their own backends which enables tight integration between AMGCL and the user code.

%In~\cite{DBLP:conf/pldi/DubachCRBF12}, 
Dubach \etal propose a new Java compatible object-oriented programming language (\texttt{Lime})~\cite{DBLP:conf/pldi/DubachCRBF12}. 
It uses high-level abstractions to explicitly represent parallelism and computation. 
The backend compiler and runtime can automatically manage the data mapping and generate OpenCL/CUDA code for GPUs. 
\texttt{Halide} is a new language for generating efficient image processing code 
on heterogeneous platforms and simplifying programming~\cite{DBLP:conf/pldi/Ragan-KelleyBAPDA13, DBLP:journals/tog/Ragan-KelleyAPLAD12}. 
Its frontend is embedded in C++, while its backend includes x86, ARMv7, CUDA and OpenCL. 
Equally used in image processing, 
\texttt{KernelGenius} is a high-level programming tool 
for EMM (explicitly managed memory many cores)~\cite{DBLP:conf/cases/LepleyPF13}. 
\texttt{Membarth} has implemented a source-to-source compiler, which translates a high-level description 
into low-level GPU codes (OpenCL, CUDA or renderscript)~\cite{DBLP:conf/ipps/MembarthHTKE12, DBLP:journals/tpds/MembarthRHTKE16}. 
Sidelnik \etal have proposed to implement a high-level programming language, \texttt{Chapel}, 
for controlling task allocation, communication and data locality structure on multi-core CPUs and GPUs.
A program in \texttt{Chapel} can run on multiple platforms, and achieve the same performance as CUDA programs~\cite{DBLP:conf/ipps/SidelnikMCGP12}. 
Hong \etal describe \texttt{Green-Marl}, a domain-specific language,
whose high-level language constructs allow developers to describe their graph analysis algorithms intuitively, 
but expose the data-level parallelism inherent in the algorithms~\cite{DBLP:conf/asplos/HongCSO12}. 
%The domain-specific programming model is built on a compiler, 
%which translates high-level algorithmic description written 
%in Green-Marl into an efficient C++ implementation by exploiting 
%this exposed data-level parallelism. 
%In~\cite{57}, Muller \etal put forward a programming framework to enable performance portability between CPUs and accelerators.
%This framework provides users with a frontend based on FORTRAN language extension, 
%and can convert a unified representation into standard x86 FORTRAN or FORTRAN with OpenACC.

The deep learning frameworks (e.g., \texttt{Tensorflow}~\cite{DBLP:journals/corr/AbadiABBCCCDDDG16}, \texttt{PyTorch}~\cite{DBLP:conf/nips/PaszkeGMLBCKLGA19}, 
and \texttt{MXNet}~\cite{DBLP:journals/corr/ChenLLLWWXXZZ15}) 
provide users with script or functional languages (e.g., \textit{Python}, \textit{R}, \textit{Scala}, \textit{Julia}) in the frontend.
These script languages are used to describe the workflow of training or inference.
At the backend, the frameworks dispatch tasks to the underlying heterogeneous systems (GPUs or FPGAs) 
via low-level or other high-level programming models such as OpenCL, CUDA or SYCL.
%programming models in the back end For the underlying heterogeneous computing devices such as GPU and FPGA, 
This whole process of mapping tasks is transparent to users.
%~\cite{DBLP:journals/corr/AbadiABBCCCDDDG16}.

To sum up, the domain-specific programming models have the potential to improve programmer productivity, 
to support domain-specific forms of modularity, and to use domain-specific information to support optimizations~\cite{DBLP:journals/tog/MarkGAK03}.
Most of these advantages are obtained by raising the language's abstraction level with domain-speciﬁc data types, operators, and control constructs.
Although the domain-specific programming models can generate efficient kernel code, they are limited to specific application domains. 
%And they are often built upon the high-/low-level programming models. 






==> pp-models - Copy/ext.tex <==
%\subsection{Extending Programming Models for Multiple Devices}
\vspace{-2mm}
\subsection{Supporting Multiple Devices}
%Multi-accelerator systems are the natural target platform for the GPUSs framework. 
%A generic multi-accelerator system consists of a general-purpose processor
%(possibly with several cores) 
%called host, connected to a number of hardware accelerators, or devices. 
%We assume that each device can only access its own local memory space. 
%In our case, the devices are programmable GPUs which communicate with the CPU via a PCIExpress bus. 
%Direct communication between devices is not possible, so that data transfer between them must be performed
%through the host memory (main memory).

%While general-purpose homogeneous multi-core architectures are becoming ubiquitous, there are clear indications that, 
%for a number of important applications, a better performance/power ratio can be attained using specialized hardware accelerators. 
%These accelerators require specific SDK or programming languages which are not always easy to program. 
%Thus, the impact of the new programming paradigms on the programmer's productivity will determine their success 
%in the high-performance computing arena. 

The interest in using multiple 
%graphics processing units (GPUs) 
accelerating devices
to speed up applications 
has increased in recent years. However, the existing heterogeneous programming models (e.g., OpenCL) 
abstract details of devices at the per-device level and 
require programmers to explicitly schedule their kernel tasks on a system 
equipped with multiple devices. 
%Unfortunately, multiple applications running on a multi-GPU system may 
%compete for some of the GPU devices while leaving other GPU devices unused. 
%Moreover, the distributed memory model defined in OpenCL, 
%where each device has its own memory space, 
%increases the complexity of managing the memory among multiple GPU devices. 
%In this subsection, we review the techniques of extending parallel programming models to support multiple devices. 
This subsection examines the software techniques of extending parallel programming models to support multiple devices. 

%Computational accelerators, such as manycore NVIDIA GPUs, Intel Xeon Phi and FPGAs, 
%are becoming common in work-stations, servers and supercomputers 
%for scientific and engineering applications. 
%Efficiently exploiting the massive parallelism these accelerators provide requires the designs and implementations of productive programming models. 

\cparagraph{GPUSs} 
%Ayguad{\'{e}} \etal present GPU Superscalar (GPUSs), an extension of the Star Superscalar programming model 
The GPU Superscalar (\texttt{GPUSs}) is an extension of the Star Superscalar (\texttt{StarSs}) programming model 
that targets application parallelization on platforms 
%consisting of a general-purpose processor connected 
with multiple GPUs~\cite{DBLP:conf/europar/AyguadeBILMQ09}. 
%GPUSs 
This framework deals with architecture heterogeneity and 
%separate memory address spaces, 
separate memory spaces, 
while preserving simplicity and portability. 
%Preliminary experimental results for a well-known operation in numerical linear algebra illustrate 
%the correct adaptation of the runtime to a multi-GPU system, 
%attaining notable performance results.

\cparagraph{VirtCL}
You \etal propose a framework (\texttt{VirtCL}) that reduces the programming burden by acting as a layer 
between the programmer and the native OpenCL run-time system.
\texttt{VirtCL} abstracts multiple devices into a single virtual device~\cite{DBLP:conf/ppopp/YouWTC15}.
%and for scheduling computations and 
%communications among the multiple devices~\cite{DBLP:conf/ppopp/YouWTC15}. 
This framework comprises two main software components: a front-end library, 
which exposes primary OpenCL APIs 
and the virtual device, and  a back-end run-time system (CLDaemon) for 
scheduling and dispatching kernel tasks based on a history-based scheduler. 
%The front-end library forwards computation requests to the back-end CLDaemon, 
%which then schedules and dispatches the requests. 
%We also propose a history-based scheduler that is able to schedule kernel tasks in a contention- and communication-aware manner. 
%Experiments demonstrated that the VirtCL framework introduced a small overhead (mean of 6\%) 
%but outperformed the native OpenCL run-time system for most benchmarks in the Rodinia benchmark suite,
%which was due to the abstraction layer eliminating the time-consuming initialization of OpenCL contexts. 
%We also evaluated different scheduling policies in VirtCL with a real-world application (clsurf) and 
%various synthetic workload traces. The results indicated that the VirtCL framework provides scalability for multiple kernel tasks running on multi-GPU systems.

\cparagraph{OpenMP extension}
Yan \etal explore support of multiple accelerators in high-level programming models 
%by designing language extensions to OpenMP to support offloading data and computation regions 
by extending OpenMP to support offloading data and computation regions 
to multiple accelerators~\cite{DBLP:conf/ppopp/0001LLSQ15}. 
These extensions allow for distributing data and computation among a list of devices via easy-to-use interfaces, 
including specifying the distribution of multi-dimensional arrays and 
%declaring shared data regions among accelerators. 
declaring shared data regions. 
%Computation distribution is realized by partitioning a loop iteration space among accelerators. We implement mechanisms to marshal/unmarshal and to move data of non-contiguous array subregions and shared regions between accelerators without involving CPUs. We design reduction techniques that work across multiple accelerators. Combined compiler and runtime support is designed to manage multiple GPUs using asynchronous operations and threading mechanisms. We implement our solutions for NVIDIA GPUs and demonstrate through example OpenMP codes the effectiveness of our solutions for performance improvement.

%\cparagraph{OpenMP+OpenACC}~\cite{DBLP:journals/sp/XuTCC15}
%Existing studies show that using single GPU can lead to obtaining significant performance gains. We should be able to achieve further performance speedup if we use more than one GPU. Heterogeneous processors consisting of multiple CPUs and GPUs offer immense potential and are often considered as a leading candidate for porting complex scientific applications. Unfortunately programming heterogeneous systems requires more effort than what is required for traditional multicore systems. Directive-based programming approaches are being widely adopted since they make it easy to use/port/maintain application code. OpenMP and OpenACC are two popular models used to port applications to accelerators. However, neither of the models provides support for multiple GPUs. A plausible solution is to use combination of OpenMP and OpenACC that forms a hybrid model; however, building this model has its own limitations due to lack of necessary compilers' support. Moreover, the model also lacks support for direct device-to-device communication. To overcome these limitations, an alternate strategy is to extend OpenACC by proposing and developing extensions that follow a task-based implementation for supporting multiple GPUs. We critically analyze the applicability of the hybrid model approach and evaluate the proposed strategy using several case studies and demonstrate their effectiveness.


\cparagraph{OpenACC-to-CUDA}                                                                                                                                                     %Although early evaluations of the OpenACC systems showed significant performance improvement with modest programming efforts,
%they also revealed the limitations of the systems.
%One of the biggest limitations is that the current OpenACC compilers do not
%automate the utilization of multiple GPUs.
%In this paper, we 
Komoda \etal present an OpenACC compiler 
%with the capability to execute single 
to run single OpenACC programs on multiple GPUs~\cite{DBLP:conf/icpp/KomodaMNM13}.
By orchestrating the compiler and the runtime system, 
the proposed system can efficiently manage the necessary data movements 
among multiple GPUs memories. 
%To enable advanced communication optimizations, 
%the authors propose a small set of directives as extensions of OpenACC API. 
The authors extend a set of directives based on the standard OpenACC API to facilitate communication optimizations. 
The directives allow programmers to express the patterns of memory accesses in the parallel loops to be offloaded. 
Inserting a few directives into an OpenACC program can reduce a large amount of unnecessary data movements.
%and thus helps the proposed system drawing great performance from multi-GPU systems. 
%We implemented and evaluated the prototype system on top of CUDA with three data parallel applications. The proposed system achieves up to 6.75x of the performance compared to OpenMP in the 1CPU with 2GPU machine, and up to 2.95x of the performance compared to OpenMP in the 2CPU with 3GPU machine. In addition, in two of the three applications, the multi-GPU OpenACC compiler outperforms the single GPU system where hand-written CUDA programs run.


==> pp-models - Copy/high.tex <==
\subsection{High-level Parallel Programming Models} \label{sec:highlevel-ppm}
To lower programming barrier,
%researchers have put forward various strategies to improve the abstraction level,
various strategies have been proposed to improve the abstraction level,
i.e., high-level programming models.
This is achieved by redefining programmers' role
%the boundary between programmers and programming systems
 and
letting compilers and runtime systems take more work.
Ultimately, the high-level parallel programming models aim to
free programmers from mastering the low-level APIs
or performing architecture-specific optimizations.
There are five types of high-level programming models:
(1) the C++-based programming models,
%general heterogeneous programming model based on C++,
(2) the skeleton-based programming models,
%standard template library Or the programming model of the algorithm pattern library,
(3) the STL-based programming models,
%(3) the programming model based on the compilation guidance command,
(4) the directive-based programming models, and
(5) the domain-specific programming models.
%(4) the feature oriented Domain specific programming model.


\subsubsection{C++-based Programming Models}
SYCL is a cross-platform abstraction layer that builds on OpenCL's concepts, portability and efficiency for programming heterogeneous platforms
in a single-source style with standard C++.
%Different from OpenCL, SYCL
This programming model enables the host and kernel code
for an application to be contained in the same source file,
%in a type-safe way and with
and achieves the simplicity of a cross-platform asynchronous task graph~\cite{sycl-spec}.
Intel has been developing oneAPI that includes DPC++ (an implementation of SYCL with extensions) for its CPUs, GPUs and FPGAs~\cite{oneapi_url}.
%With the additional support for SYCL from Xilinx, Renesas and Imagination Technologies, software developers are now
%SYCL is not able to target a wide range of devices using SYCL.
C++ AMP (C++ Accelerated Massive Parallelism) is a heterogeneous programming model based on C++.
% and runtime library.
Built upon DirectX11, this model uses \textit{parallel\_for\_each} to instantiate device code, and provides users with a C++ programming interface.
%In this way,
Thus, the programmer can write GPU code in a more concise and controlled way~\cite{amp_book}.
Inspired by C++ AMP and C++14, HC (Heterogeneous Computing) C++ API is a GPU-oriented C++ compiler developed by AMD~\cite{hcc_url}.
%Different from C++ AMP,
HC removes the ``restrict'' keyword,
supports additional data types in kernels, and
provides fine-grained control over synchronization and data movement.
%HC is designed to expose cutting edge compute capabilities on Boltzmann and HSA devices to developers while offering the productivity and usability of C++.
%SYCL includes templates and generic lambda functions to enable higher-level application software
%to be cleanly coded with optimized acceleration of kernel code across the extensive range of shipping OpenCL 1.2 implementations.
%Developers program at a higher level than OpenCL C or C++,
%but always have access to lower-level code through seamless integration with OpenCL,
%C/C++ libraries, and frameworks such as OpenCV or OpenMP.

\texttt{PACXX} is a unified programming model for programming heterogeneous many-core systems,
to mitigate the issue of long, poorly structured and error-prone codes in low-level programming models~\cite{DBLP:conf/sc/HaidlG14}.
In PACXX, both host and device programs are written in the
%same programming language – the newest
C++14 standard,
with all modern C++ features including type inference (auto),
variadic templates, generic lambda expressions, as well as
STL containers and algorithms.
%Figure~\ref{fig:pacxx-sw-stack} shows that
PACXX consists of a custom compiler (based on the Clang front-end and
LLVM IR) and a runtime system,
%which work together to
which facilitate automatic memory management and data synchronization~\cite{DBLP:journals/ijpp/HaidlG18, DBLP:conf/sc/HaidlMKSHG17}.
% automatically
%and
%which is transparent to programmers~\cite{DBLP:journals/ijpp/HaidlG18}.


Other C++-based parallel programming models include boost.compute~\cite{DBLP:conf/iwocl/Szuppe16},
HPL~\cite{DBLP:journals/jpdc/VinasBF13, DBLP:journals/concurrency/VinasFAD18}, VexCL~\cite{denis_demidov_2017_571466},
hlslib for FPGAs~\cite{DBLP:journals/corr/abs-1910-04436}, alpaka~\cite{DBLP:conf/ipps/ZenkerWWHJKNB16}, and so on.
%With the help of modern C++,
By respecting the philosophy of modern C++,
these high-level programming models integrate
the host code and the device code into a single C++ file,
and use a unified data structure to manage the buffer to avoid manual management of data synchronization.
% without the need for
By doing so, programmers can transparently use the parallel computing resources of many-core architectures,
without having to master their details.
% of the underlying processor architecture.
%so that they can transparently use the parallel computing resources of multi-core processors,
%be compatible with programming simplicity and code portability.
An important feature of the C++-based parallel programming model is that,
it can form a natural match with other C++ programs, which facilitates the development and composition of
large-scale scientific computing applications, significantly improving programmability and productivity.
%The combination of software modules improves the programmability and programming productivity.


%\biegin{figure}[!t]
%  %\centering
%  \includegraphics[width=0.48\textwidth]{fig/pacxx.png}
%  \caption{The architecture of PACXX~\cite{DBLP:conf/sc/HaidlMKSHG17}.}
%  \label{fig:pacxx-sw-stack}
%\end{figure}
\subsubsection{Skeleton-based Programming Models\label{sec:skeleton}}

Skeleton programming is a programming paradigm based on algorithmic skeleton~\cite{skeleton_book}.
A skeleton is a predefined ``high-order function'', such as \textit{map}, \textit{reduce}, \textit{scan}, \textit{farm}, and \textit{pipeline},
which implements a common pattern of computation and/or data dependence.
%a kind of public computing or communication pattern.
%It takes user-defined code as input instantiation as a specific function, such as map, reduce, scan, farm, pipeline, etc.
Skeleton programming provides a high level of abstraction and portability,
with a quasi-sequential programming interface,
as their implementations encapsulate all the underlying details and architecture features,
including parallelization, synchronization, communication, buffer management, accelerator usage and many others.

%Skeleton programming is an approach where an application is written with the help of skeletons.
%A skeleton is a pre-defined, generic component such as map, reduce, scan, farm, pipeline etc. that implements a common specific pattern of computation and data dependence, and that can be customized with (sequential) user-defined code parameters. Skeletons provide a high degree of abstraction and portability with a quasi-sequential programming interface, as their implementations encapsulate all low-level and platform-specific details such as parallelization, synchronization, communication, memory management, accelerator usage and other optimizations.

SkePU is a skeleton programming framework based on the C++ template for multi-core CPU and multi-GPU systems.
This framework contains six data-parallel and one task-parallel skeletons, and two generic container types.
The backend support of SkePU includes OpenMP, OpenCL and CUDA,
where Clang is used to facilitate the source-to-source
code transformation~\cite{DBLP:conf/appt/DastgeerLK13}.
The interface of SkePU2 is improved based on C++11 and variadic templates,
and user-defined functions are expressed with the lambda expression~\cite{DBLP:journals/ijpp/ErnstssonLK18}.

SkelCL is another skeleton library for heterogeneous platforms~\cite{DBLP:conf/ipps/SteuwerKG11}.
It provides programmers with vector data type, high-level data distribution mechanism to
enable the automatic buffer management, implicit data transfers between host and accelerator.
This aims to significantly simplify the programming of heterogeneous many-core systems.
The SkelCL backend translates each skeleton into an OpenCL kernel, and
enables the SkelCL codes to run on both multi-core CPUs and heterogeneous GPUs.
This framework also supports automatic mapping of tasks onto multiple devices~\cite{DBLP:journals/tjs/SteuwerG14}.

Other skeleton-based programming models include Muesli~\cite{muesli_techreport}, Marrow~\cite{DBLP:conf/europar/MarquesPAM13},
ParallelME~\cite{DBLP:conf/europar/AndradeCUCAFRFG16, DBLP:conf/sbac-pad/MoreiraACGFRSA17}, etc.
Compared with the C++-based programming models, the skeleton programming model is lack of generality,
i.e.,  some computing or communication patterns are difficult to be represented
by the builtin skeletons.
Thus we have to extend the existing skeletons
%make a lot of extension
when necessary.
%For a given application,
Programmers are also responsible for synthesizing their target applications with builtin skeletons.

%\cparagraph{ParallelME}
%Andrade \etal present ParallelME~\cite{DBLP:conf/europar/AndradeCUCAFRFG16, DBLP:conf/sbac-pad/MoreiraACGFRSA17},
%aims to produce high-performance code with low-energy consumption.
%ParallelME automatically coordinates the parallel
%usage of computing resources keeping the programming
%effort similar to what sequential programmers expect.
%ParallelME offers a programming abstraction (i.e. patterns)
%in Java that can be used by Android developers to
%produce parallel code in low-level frameworks with
%minimum effort.
%ParallelME singles itself from other frameworks
%by its high-level programming abstraction in Java and the
%ability to efficiently coordinate resources in heterogeneous
%mobile architectures. This is achieved through a source-to-source
%%compiler that translates the high-level operations
%in Java to low-level tasks that are coordinated during
%execution by OpenCL or RenderScript.

\subsubsection{STL-based Programming Models}
TBB (Threading Building Blocks) is a C++ template library developed by Intel for parallel programming of its multi-core CPUs.
It implements a set of algorithm components (e.g., \textit{parallel\_for}, \textit{parallel\_reduce}) and
a set of containers (e.g., \textit{concurrent\_queue}, \textit{concurrent\_vector}).
The TBB runtime system is responsible for managing and scheduling threads to execute tasks, and
balancing the computing loads between multi-cores by task stealing.
By doing so, TBB aims to unbind programmers and the underlying hardware~\cite{DBLP:journals/software/KimV11}.
HPX (High Performance ParallelX) is a generic C++ runtime system for parallel and distributed systems~\cite{hpx_su, DBLP:conf/sc/HellerKSF13}.
%communication that can face any scale of parallel and distributed systems
%Using C + + runtime system [38].
By providing a unified programming interface,
HPX can transparently use the underlying hardware resources with an asynchronous multi-tasking mechanism.
HPX aims to be easy-to-use, and achieves high scalability and portability.
HPX enables the support of heterogeneous computing,
by introducing the concepts of \textit{target}, \textit{allocator} and \textit{executor} within the \texttt{hpx.compute} subproject.
The backend of the computing platform includes CUDA, HCC and SYCL~\cite{DBLP:conf/iwocl/CopikK17, DBLP:conf/supercomputer/HellerKDFS16}.

Thrust is a C++ standard parallel template library for NVIDIA GPUs.
It implements four basic core algorithms for \textit{each}, \textit{reduce}, \textit{scan} and \textit{sort}~\cite{BELL2012359}.
By doing so, users need not know how to map the calculation to the computing resources
 (e.g., thread block size, buffer management, algorithm variant selection, etc.),
but only pay attention to the calculation itself.
This approach can greatly improve productivity.
%This programming approach can greatly ensure the programming efficiency of programmers.
Thrust's backend is based on CUDA, TBB, and OpenMP.
%Microsoft's PPL (Parallel Patterns Library) is a template library for multi-core platform similar to C++ standard template library.
%Built on Windows' ThreadPool, PPL provides a general, type safe parallel algorithm and a container for concurrent data processing,
%which can improve the application scalability and simplify the program development process~\cite{ppl_url}.
% is simplified while the application scalability is improved [42].
Kokkos
%C++ ecosystem is a production-level solution
allows programmers to write modern C++ applications in a hardware-agnostic manner~\cite{DBLP:journals/jpdc/EdwardsTS14}.
It is a programming model for parallel algorithms that use many-core chips and share memory among those cores.
%(Figure~\ref{fig:kokkos-sw-stack}).
%part of the U.S. Department of Energy's Exascale Computing Project, shown in Figure~\ref{fig:kokkos-sw-stack},
%a national effort to prepare the HPC community for the next generation of supercomputing platforms~\cite{DBLP:journals/jpdc/EdwardsTS14}.
%With this framework, Kokkos Core is a programming model for parallel algorithms that use many-core chips and share memory among those cores.
This programming model includes computation abstractions for frequently used parallel computing patterns, policies that provide details for how those computing patterns are applied, and execution spaces that denote on which cores the parallel computation is performed.

%The programming model also includes patterns for common data structures, policies that provide details for how those data structures are laid out in memory, and memory spaces that denote in which memory the data reside.
%The Kokkos Core programming model works by requiring that application development teams implement their algorithms in terms of Kokkos' patterns, policies, and spaces. Kokkos Core can then map these algorithms onto the target architecture according to architecture-specific rules necessary to achieve best performance. While other programming models support execution patterns, execution policies, execution spaces, and memory spaces; only Kokkos supports data patterns and policies, which are necessary for performance portability.

%\begin{figure}[!t]
%  %\centering
%  \includegraphics[width=0.45\textwidth]{fig/kokkos.png}
%  \caption{The Kokkos C++ performance portability ecosystem for exascale systems~\cite{DBLP:journals/jpdc/EdwardsTS14}.}
%  \label{fig:kokkos-sw-stack}
%\end{figure}

Other similar STL-based programming models include
%Kokkos~\cite{DBLP:journals/jpdc/EdwardsTS14},
Microsoft's PPL (Parallel Patterns Library)~\cite{ppl_url},
RAJA~\cite{DBLP:conf/ppopp/BeckingsaleHSV19}, etc.
This kind of programming model implements the functions and their extensions in the standard C++ template library,
and provides concurrent data structures.
%By doing so,
% that supports parallel access, and
Thus, this programming model can unbind the parallel programming itself with the underlying hardware resources.
%Therefore, with these programming models,
Programmers do not need to care about the details of the underlying architectures,
which effectively lowers the programming barrier.
%The problem of STL-based programming model is that it can only call fixed format library function,
%but modern C++ STL is becoming increasingly more general.
%Therefore, this project classifies the programming model based on standard template library and the programming model based on pattern algorithm library into one class.



\subsubsection{Directive-based Programming Models}
Another high-level programming models are based on directive annotations,
%e.g. OpenMP~\cite{omp_url}, OpenACC~\cite{oacc_url}, OmpSs~\cite{DBLP:journals/ppl/DuranABLMMP11},
%XcalableMP~\cite{DBLP:conf/ipps/NomizuTLBS12}, Intel LEO~\cite{mpss_url}, and Mint~\cite{DBLP:conf/ics/UnatCB11}.
including both industry standardards (OpenMP~\cite{omp_url}, OpenACC~\cite{oacc_url}, Intel LEO~\cite{mpss_url}) and
academia-maintained efforts (OmpSs~\cite{DBLP:journals/ppl/DuranABLMMP11},
XcalableMP~\cite{DBLP:conf/ipps/NomizuTLBS12}, Mint~\cite{DBLP:conf/ics/UnatCB11}, OpenMDSP~\cite{DBLP:conf/IEEEpact/HeCCZTY11}).
These programming models only have to add directive constructs before the target code region,
while the tasks of offloading, parallelization and optimization are delegated to compilers and runtime systems.
%compilation guidance statements in front of the target area,
%while the parallelization and optimization work is the responsibility of the back-end compiler and runtime environment.
On one hand, programmers do not have to master a large number of architectural details, thus leading to an improved productivity.
On the other hand, programmers can annotate their codes incrementally, which also lowers the barrier of debugging.
Therefore, this programming model enables the non-experts to enjoy the performance benefits of
heterogeneous many-cores without being entangled in the architecture details.

%One directive-based programming can be mapped onto multiple many-core architectures.
Multiple directive-based programming models can be mapped onto a single many-core architecture.
%\cparagraph{CellSs/OpenMP on Cell/B.E.}
As we have mentioned in Section~\ref{subsec:vendor-ppm}, programming the Cell/B.E. processor is challenging.
There is a significant amount of research in programming models that
attempts to make it easy to exploit the computation power of the CEBA architecture.
%To achieve the simplicity and flexibility of the programming model,
Bellens \etal present Cell superscalar (CellSs)
which addresses the automatic exploitation of the functional parallelism of a sequential program
through the different processing elements of the CEBA architecture~\cite{DBLP:conf/sc/BellensPBL06}.
Based on annotating the source code, a source-to-source compiler generates the necessary code and a runtime library
exploits the existing parallelism by building a task dependency graph.
% during runtime.
The runtime takes care of task scheduling and data movements between the different processors of this architecture.
O'Brien \etal explore supporting OpenMP on the Cell processor~\cite{DBLP:journals/ijpp/OBrienOSCZ08} based on IBM's XL compiler,
so that programmers can continue using their familiar programming model and existing code can be re-used.

%It is attractive to support OpenMP because programmers can continue using their familiar
%programming model, and existing code can be re-used. The authors base our work on IBM's
%XL compiler, and developed new components in the XL compiler and a new runtime
%library. Three major issues are addressed: (1) synchronization support on heterogeneous cores;
%(2) code generation targeting the different instruction sets;
%(3) data transfers and implement the OpenMP memory model. They present experimental results for
%some SPEC OMP 2001 and NAS benchmarks to demonstrate the effectiveness of this
%approach. A visualization tool based on Paraver is also used to provide some insights
%into actual thread and synchronization behaviors.

%\cparagraph{CellSs on Cell}
%In~\cite{DBLP:conf/sc/BellensPBL06}, Bellens \etal present Cell superscalar (CellSs) which addresses the automatic exploitation of the functional parallelism
%of a sequential program through the different processing elements of the Cell BE architecture.
%The focus in on the simplicity and flexibility of the programming model.
%Based on a simple annotation of the source code, a source to source compiler generates the necessary code and a runtime library
%exploits the existing parallelism by building at runtime a task dependency graph.
%The runtime takes care of the task scheduling and data handling between the different processors of this heterogeneous architecture.
%Besides, a locality-aware task scheduling has been implemented to reduce the overhead of data transfers.
%The approach has been implemented and tested with a set of examples and the results obtained since now are promising.

%\cparagraph{Mint on CUDA}
%We present Mint, a programming model that enables the non-expert to enjoy the performance benefits of
%hand coded CUDA without becoming entangled in the details~\cite{DBLP:conf/ics/UnatCB11}.
%Mint targets stencil methods, which are an important class of scientific applications.
%We have implemented the Mint programming model with a source-to-source translator that
%generates optimized CUDA C from traditional C source.
%The translator relies on annotations to guide translation at a high level.
%The set of pragmas is small, and the model is compact and simple.
%Yet, Mint is able to deliver performance competitive with painstakingly hand-optimized CUDA.
%We show that, for a set of widely used stencil kernels, Mint realized 80\% of the performance
%obtained from aggressively optimized CUDA on the 200 series NVIDIA GPUs.
%Our optimizations target three dimensional kernels,
%which present a daunting array of optimizations.


==> pp-models - Copy/intro.tex <==
\section{Introduction}

%\begin{itemize}
%\item High performance computing systems is made from heterogeneous many-core architectures.

%\item Programming such systems is challenging due to (1) heterogenisity, (2) many-cores, (3) complex memory herarchy.

%\item Recently, researchers have proposed parallel programming models for such systems: low-level programming models and high-level programming models.

%\item However, none programming models have become the de facto standard.

%\item predicting future trends? A new programming system?? this is a test

%\end{itemize}

Heterogeneous many-core systems are now commonplace~\cite{DBLP:conf/eurographics/OwensLGHKLP05, DBLP:journals/pieee/OwensHLGSP08}. The
combination of using a host CPU together with specialized processing units (e.g., GPGPUs, XeonPhis, FPGAs, DSPs and NPUs) has been shown in
many cases to achieve orders of magnitude performance improvement. 
As a recent example, Google's Tensor Processing Units (TPUs) are application-specific integrated circuits (ASICs) 
to accelerate machine learning workloads~\cite{DBLP:conf/isscc/Patterson18}. 
Typically, the host CPU of a heterogeneous platform manages the
execution context while the computation is offloaded to the accelerator or coprocessor. Effectively leveraging such platforms not only
enables the achievement of high performance, but increases energy efficiency. These goals are largely achieved using simple, yet
customized hardware cores that use area more efficiently with less power dissipation~\cite{DBLP:journals/ibmrd/ChenRDI07}.


The increasing importance of heterogeneous many-core architectures can be seen from the TOP500 and Green500 list, where a large number of
supercomputers are using both CPUs and accelerators~\cite{top500_url, green500_url}. A closer look at the list of the TOP500
supercomputers shows that seven out of the top ten supercomputers are built upon heterogeneous many-core architectures
(Table~\ref{tab:sc-top10-ppm}). On the other hand, this form of many-core architectures is being taken as building blocks for the
next-generation supercomputers. 
%For example, to deliver US's exascale supercomputing systems,
%in the 2021-2023 timeframe, 
e.g., three US national projects (Aurora~\cite{aurora_url}, Frontier~\cite{frontier_url}, and El Capitan~\cite{capitan_url}) will all implement a
heterogeneous CPU-GPU architecture to deliver its exascale supercomputing systems.


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[]
%\centering
\caption{The on-node parallel programming models for the top10 supercomputers (as of November 2019).}
\label{tab:sc-top10-ppm}
\resizebox{0.70\textwidth}{!}{%
\begin{tabular}{@{}lclcc@{}}
\toprule
\textbf{Rank} &
  \textbf{Name} &
  \textbf{Compute node architecture} &
  \textbf{Heterogeneous?} &
  \textbf{Programming models} \\ \midrule
\#1 &
  Summit &
  \begin{tabular}[c]{@{}l@{}}IBM POWER9 22C CPU (x2)+\\ NVIDIA Volta GV100 (x6)\end{tabular} &
  YES &
  CUDA/OpenMP \\
\rowcolor[HTML]{C0C0C0}
\#2 &
  Sierra &
  \begin{tabular}[c]{@{}l@{}}IBM POWER9 22C CPU (x2)+\\ NVIDIA Volta GV100 (x4)\end{tabular} &
  YES &
  CUDA/OpenMP \\
\#3 &
  TaihuLight &
  Sunway SW26010 260C &
  YES &
  Athread/OpenACC \\
\rowcolor[HTML]{C0C0C0}
\#4 & Tianhe-2A & \begin{tabular}[c]{@{}l@{}}Intel Xeon E5-2692v2 12C CPU (x2)+\\ Matrix-2000 (x2)\end{tabular}            & YES & OpenCL/OpenMP \\
\#5 &
  Frontera &
  Xeon Platinum 8280 28C CPU &
  NO &
  OpenMP \\
\rowcolor[HTML]{C0C0C0}
\#6 &
  Piz Daint &
  \begin{tabular}[c]{@{}l@{}}Xeon E5-2690v3 12C CPU (x1)+\\ NVIDIA Tesla P100 (x1)\end{tabular} &
  YES &
  CUDA \\
\#7 &
  Trinity &
  \begin{tabular}[c]{@{}l@{}}Intel Xeon E5-2698v3 16C CPU \& \\ Intel Xeon Phi 7250 68C\end{tabular} &
  NO &
  OpenMP \\
\rowcolor[HTML]{C0C0C0}
\#8 & ABCI      & \begin{tabular}[c]{@{}l@{}}Intel Xeon Gold 6148 20C CPU (x2)+\\ NVIDIA Tesla V100 SXM2 (x4)\end{tabular} & YES & CUDA          \\
\#9 &
  SuperMUC-NG &
  Intel Xeon Platinum 8174 24C CPU &
  NO &
  OpenMP \\
\rowcolor[HTML]{C0C0C0}
\#10 &
  Lassen &
  \begin{tabular}[c]{@{}l@{}}IBM POWER9 22C CPU (x2)+\\ NVIDIA Tesla V100 (x4)\end{tabular} &
  YES &
  CUDA/OpenMP \\ \bottomrule
\end{tabular}%
}
\end{table*}


The performance of heterogeneous many-core processors offer a great deal of promise for future computing systems, yet their architecture
and programming model significantly differ from the conventional multi-core processors~\cite{DBLP:conf/sc/BellensPBL06}. This change has
shifted the burden onto programmers and compilers~\cite{DBLP:conf/pldi/KudlurM08}. In particular, programmers have to deal with
heterogeneity, massive processing cores, and a complex memory hierarchy. Thus, programming heterogeneous many-core architectures are
extremely challenging.
%All these actions are enabled with the help of parallel programming models.


How to program parallel machines has been a subject of research for at least four decades~\cite{karp1967organization}. The main contextual
difference between now and the late 80s/early 90s is that heterogeneous parallel processing will be shortly a mainstream activity affecting
standard programmers rather than a high-end elite endeavour performed by expert programmers. This changes the focus from one where raw
performance was paramount to one where programmer productivity is critical. In such an environment, software development tools and
programming models that can reduce programmer effort will be of considerable importance.


In this work, we aim to demystify heterogeneous computing and show heterogeneous parallel programming is a trustworthy and exciting
direction for systems research. We start by reviewing the historical development and the state-of-the-art of parallel programming models for heterogeneous many-cores by
examining solutions targeted at both low-level and high-level programming (Section~\ref{sec:overview}). We then discuss code generation
techniques employed by programming models for improving programmability and/or portability (Section~\ref{sec:bridge}), before turning our
attention to software techniques for optimizing the communication overhead among heterogeneous computing devices (Section~\ref{sec:stream}).
Finally, we outline the potential research directions of heterogeneous parallel programming models (Section~\ref{sec:next}).

%In this article, we review the state-of-the-art of parallel programming models for heterogeneous many-core architectures, and categorize
%them into low-level models and high-level models (Section~\ref{sec:overview}). Then, we examine the code generation techniques between
%programming models for improving programmability and/or portability (Section~\ref{sec:bridge}). We also review the techniques of optimizing
%host-accelerator communications (Section~\ref{sec:stream}). At last, we give a perspective of the development of parallel programming
%models in the future (Section~\ref{sec:next}).

%This survey stands out in (1) we focus on the parallel programming models for heterogeneous many-cores~\cite{DBLP:journals/tpds/DiazMN12} (2) (3)


==> pp-models - Copy/low.tex <==
\subsection{Low-level Parallel Programming Models} \label{sec:lowlevel-ppm}
\vspace{-2mm}
\subsubsection{Prelude of GPGPU Programming}
%\subsubsection{The Prelude of Heterogeneous Computing and Programming}
\vspace{-2mm}
\textbf{The GPU Shading Lanuages} At early 2000s, commodity graphics hardware was rapidly evolving from a fixed function pipeline into
a programmable vertex and fragment processor.
Originally, these programmable GPUs could only be programmed using assembly language.
Later, Microsoft and NVIDIA introduced their C-like programming languages, HLSL and Cg respectively, that compile to
GPU assembly language~\cite{hlsl_url, DBLP:journals/tog/MarkGAK03}.
The shading languages make it easier to develop programs incrementally and interactively.
This is achieved by using a high-level shading language, e.g., Cg, based on both the syntax and the philosophy of C.
%[Kernighan and Ritchie 1988].
%GPU shading languages: Cg, HLSL, GLSL

%Such high-level languages provide the usual benefits of program portability and improved programmer productivity,
%and they also make it easier develop programs incrementally and
%interactively, a benefit that is particularly valuable for shader programs.
%%This can be achieved by designing the high-level shading languages, e.g. Cg, based on both the syntax and the philosophy of C [Kernighan and Ritchie 1988]. In particular,
%Cg is intended to be general-purpose (as much as is possible
%on graphics hardware), rather than application specific, and is
%a hardware-oriented language. As in C, most data types and operators have an obvious mapping to hardware operations, so
%that it is easy to write high-performance code.

Although these shading languages can hide details of the graphics pipeline (e.g., the number of stages or
the number of passes), they are specialized for real-time shading and remain very graphics-centric~\cite{DBLP:journals/tog/BuckFHSFHH04}.
In particular, these high-level shading languages
do not provide a clean abstraction for general-purpose computing on graphics hardware.
%(e.g. by providing light and surface shaders) and
%These languages are specialized for shading
%(e.g. by providing light and surface shaders), and hide details of the graphics pipeline such as the number of stages or
%the number of passes.
%While these high-level shading languages permit general data types
%and arbitrary user code to be executed on on graphics hardware, it remains very graphics centric and
%does not provide a clean abstraction for general purpose computing on graphics
%hardware.
Programs operate on vertices and fragments separated by a rasterization stage; memory is divided up into
textures and framebuffers; the interface between the graphics hardware and host is through a complex graphics API.
This often prevents applying the graphics hardware onto new applications.

%While this new programmability was primarily designed for real-time
%shading,
%\subsubsection{Brook for GPGPUs}
\cparagraph{Brook for GPGPUs}
%At the same time, many researchers have observed that
The graphics processors feature instruction sets
general enough to perform computation beyond the rendering domain.
%of rendering.
%GPU's capabilities extend beyond the domain of rendering.
Applications such as linear algebra operators~\cite{DBLP:journals/tog/KrugerW03},
numerical simulation~\cite{DBLP:conf/egh/HarrisBSL03},
and machine learning algorithms~\cite{DBLP:conf/icdar/SteinkrauSB05} have been ported to GPUs and achieved a remarkable speedup over traditional CPUs.
These research works demonstrate the potential of graphics hardware for more general-purpose computing tasks, i.e., GPGPUs.

%As the programmability and performance of modern GPUs continues to increase,
%many researchers have been looking to graphics hardware to solve problems previously performed on general purpose CPUs,
%now coined as \textit{GPGPU}.

%GPUs require a different computational model than
%the traditional von Neuman architecture [von Neuman 1945]
%used by conventional processors. Otherwise, GPUs will suffer from the same problems faced by modern CPUs: limited
%instruction level parallelism (ILP), excessive use of caching
%to capture locality, and diminishing cost-performance returns.

The first work to explore this idea is the \texttt{Brook} programming system~\cite{DBLP:journals/tog/BuckFHSFHH04}.
%Brook is a programming system that provides developers with a view of the GPU as a streaming coprocessor.
%The presentation of the Brook stream programming
%model for general-purpose GPU computing.
By introducing the concepts of \textit{streams}, \textit{kernels} and \textit{reduction operators},
Brook abstracts the GPU as a streaming processor. This abstraction is achieved by
virtualizing various GPU hardware features with a compiler and runtime system.
%At the language level,

The Brook language is an extension to the standard ANSI C and is designed to
incorporate the idea of data parallel computing and arithmetic intensity.
%into a familiar, efficient language.
%The general computational model, referred to as streaming, provides two main benefits over traditional conventional languages: Data Parallelism and Arithmetic Intensity.
A Brook program consists of legal C code plus syntactic extensions to denote streams and kernels.
%denote given functions as kernels.
%At the implementation level,
The Brook programming system
%compilation and runtime architecture
consists of \texttt{BRCC} and \texttt{BRT}.
\texttt{BRCC} is a source-to-source compiler which translates Brook codes (\texttt{.br}) into C++ codes (\texttt{.cpp}).
%The compiler converts Brook primatives into legal C++ syntax with the help of the BRT, Brook RunTime library.
\texttt{BRT} is a runtime software which implements the backend of the Brook primitives for target hardware.
%The BRT is a class library which presents a generic interface for the compiler to use.
%The implementation of the class methods are customized for each hardware supported by the system.
%The backend implementation is choosen at runtime based on the hardware available on the system or at request of the user.
%The backends include: DirectX9, OpenGL ARB, NVIDIA NV3x, and C++ reference.
\textit{We regard Brook as
%one of the most important landmarks
an origin work for programming GPGPUs, and
other parallel programming models for heterogeneous many-cores inherit many features from it. }


%\subsection{General Computing Languages}
\subsubsection{Vendor-Specific Programming Models} \label{subsec:vendor-ppm}
Vendor-specific programming models are bound to vendors and their manufactured hardware.
The typical heterogeneous many-core architectures include Cell/B.E., NVIDIA GPU,
AMD GPU, Intel XeonPhi, FPGA, DSP, and so on~\cite{DBLP:journals/sp/BrodtkorbDHHS10}.
Hardware vendors introduces their unique programming interfaces, which are restricted to their own products.
%which often work with their products.
%In this section, we will
This section examines each many-core architecture and its native programming models.
% CUDA for NVIDIA GPUs,
%\subsubsection{CUDA for NVIDIA GPUs}

\cparagraph{libSPE for IBM Cell Broadband Engine}
% pioneering
The Cell Broadband Engine Architecture (CEBA) and its first implementation Cell/B.E.
is a pioneering work of heterogeneous computing~\cite{DBLP:journals/ibmrd/KahleDHJMS05, DBLP:journals/micro/GschwindHFHWY06}.
%Another parallel technical roadmap of enabling heterogeneous computing is from IBM and its CEBA architecture.
Cell/B.E.~\cite{DBLP:conf/cicc/PhamBBHJKKKLMPR05} was designed by
%by a partnership of Sony, Toshiba, and IBM (STI) to be the heart of Sony's forthcoming PlayStation3 gaming system.
a collaboration effort between Sony, Toshiba, and IBM (STI),
and takes a radical departure from conventional multi-core architectures.
Instead of integrating identical commodity hardware cores, it uses a conventional high performance PowerPC core (PPE) which
controls eight simple SIMD cores (i.e., Synergistic Processing Elements, SPEs).
Each SPE contains a synergistic processing unit (SPU), a local store, and a memory flow controller (MFC).
Prior works have demonstrated
%the tremendous potential of the Cell architecture
%for scientific computations in terms of raw performance and power efficiency
that a wide variety of algorithms on the Cell/B.E. processor can achieve performance
that is equal to or significantly better than a general-purpose
processor~\cite{DBLP:conf/cf/WilliamsSOKHY06, DBLP:journals/ibmrd/ChenRDI07, DBLP:conf/hipc/BaderA07, DBLP:journals/tpds/ScarpazzaVP08}.
Its architecture variant, i.e., \texttt{PowerXCell 8i}, has been used to build the first peta-scale supercomputer,
\texttt{Roadrunner}~\cite{roadrunner_book, DBLP:conf/sc/BarkerDHKLPS08, DBLP:conf/ppopp/KistlerGBB09}.


Programming the CEBA processor is challenging~\cite{DBLP:conf/cf/CrawfordHKW08}.
IBM developed IBM SDK for Multicore Acceleration with a suite of software tools and libraries~\cite{cell_book}.
The SDK provides various levels of abstractions, ranging from the low-level management library to the high-level programming models,
%the ALF Library, and the data communication and synchronization library (DaCS),
to tap the Cell's potential.
Managing the code running on the SPEs of a CEBA-based system can be
done via the \texttt{libspe} library (SPE runtime management library) that is part of the
SDK package~\cite{cell_book}.
This library provides a standardized low-level programming interface that manages the SPE threads,
and enables communication and data transfer between PPE threads and SPEs.
%The APIs are described in Table~\ref{tab:low-level-api}
%enables application access the SPEs and
%run some of the program threads on those SPEs.
Besides, the SDK contains high-level programming frameworks to assist the development of parallel applications on this architecture.
%Similar to graphic hardware, the streaming data sets in 3D graphics, media, and broadband communications are
%example applications that run well on Cell's SPEs~\cite{cell_book}.
%To this end, Kudlur \etal present a compiler technique for planning and orchestrating
%the execution of streaming applications on the Cell platform~\cite{DBLP:conf/pldi/KudlurM08}.

\cparagraph{CUDA for NVIDIA GPUs}
NVIDIA implemented the unified shader model, where all shader units of graphics hardware
are capable of handling any type of shading tasks,
in the Tesla and its subsequent designs~\cite{csc_url}.
Since G80, NVIDIA's GPU architecture has evolved from Tesla~\cite{DBLP:journals/micro/LindholmNOM08, DBLP:conf/ispass/WongPSM10},
Fermi~\cite{nvidia-fermi-architecture-whitepaper}, Kepler~\cite{nvidia-kepler-architecture-whitepaper},
Maxwell~\cite{nvidia-maxwell-architecture-whitepaper},
Pascal~\cite{nvidia-pascal-architecture-whitepaper}, Volta~\cite{nvidia-volta-architecture-whitepaper},
to Turing~\cite{nvidia-turing-architecture-whitepaper}.
Each generation of NVIDIA's microarchitecture introduces new features
based on its previous one,
%Besides the CUDA cores,
e.g., the Volta architecture features tensor cores that have superior
deep learning performance over regular CUDA cores.


NVIDIA introduces CUDA to program its computing architecture for general-purpose computation~\cite{cuda_url}.
The CUDA programming model works with programming languages such as C, C++, and Fortran.
A CUDA program calls parallel kernels, with each executing in parallel across a set of
threads. The programmer organizes these threads in thread blocks and grids of
thread blocks. The GPU instantiates a kernel program on a grid of parallel thread blocks.
Each thread within a thread block executes an instance of the kernel, and has a thread ID
within its thread block, program counter, registers, and per-thread private memory.
%Under this programming model, GPUs consist of many processor cores,
%each of which can directly address into a global memory.
%The CUDUA kernel is XXX.
%This accessibility makes it easier for GPU experts in parallel programming to use GPU resources.
This accessibility makes it easier for us to use GPU resources.


With CUDA, NVIDIA GPUs have been used to speed up
both regular applications~\cite{DBLP:journals/pc/TomovDB10, DBLP:conf/sc/GovindarajuLDSM08}
and irregular ones~\cite{DBLP:conf/ppopp/HongKOO11, DBLP:conf/ppopp/MerrillGG12},
with an impressive performance increase over multi-core CPUs.
Nevertheless, Lee \etal argue that the performance gap can be narrowed by applying optimizations
for both CPUs and GPUs~\cite{DBLP:conf/isca/LeeKCDKNSSCHSD10}.
%Gregg and Hazelwood have
%shown that, when memory transfer times are included,
%it can take 2x--50x longer to run a kernel than the GPU processing time alone~\cite{DBLP:conf/ispass/GreggH11}.
Table~\ref{tab:sc-top10-ppm} shows that five of the top ten supercomputers use NVIDIA GPUs as the accelerators.
%We argue that the
The GPU-enabled architectures will continue
to play a key role in building future high-performance computing systems.

%When CUDA was first introduced by Nvidia, the name was an acronym for Compute Unified Device Architecture,[5]
%but Nvidia subsequently dropped the common use of the acronym.

% Brook+/HIP for AMD/ATI GPUs
%\subsubsection{Brook+/HIP for AMD GPUs}
\cparagraph{CAL/ROCm for AMD GPUs}
%Discrete GPUs and Fused GPUs (APUs).
AMD/ATI was the first to implement the unified shader model in its TeraScale design,
leveraging flexible shader processors which can be scheduled to process a variety of shader types~\cite{csc_url}.
%, thereby significantly increasing GPU throughput.
The TeraScale is based upon a very long instruction word (VLIW) architecture, in which the core executes operations in parallel.
%Following NVIDIA's SIMT design, AMD's GCN (Graphics Core Next)  and RDNA () leverage a RISC SIMD microarchitecture.
%contrasting the VLIW SIMD architecture of TeraScale.
The Graphics Core Next (GCN) architecture moved to a RISC SIMD microarchitecture,
%moved to a more programmable interleaved vector
%compute model
and introduced asynchronous computing~\cite{amd-gcn-vega-architecture-whitepaper}.
%, enabling traditional graphics and
%general-compute to work together efficiently~\cite{amd-gcn-vega-architecture-whitepaper}.
This design makes the compiler simpler and leads to a better utilization of hardware resources.
The RDNA (Radeon DNA) architecture is optimized for efficiency and programmability, while offering
backwards compatibility with the GCN architecture~\cite{amd-rdna-architecture-whitepaper}.
%A group of threads is the most basic unit of scheduling of GPUs implementing this approach to hide latency, is minimum size of the data processed in SIMD fashion, the smallest executable unit of code, the way to processes a single instruction over all of the threads in it at the same time.
As the counterpart to the gaming-focused RDNA, CDNA is AMD's compute-focused architecture for HPC and ML workloads.


Close-To-the-Metal (CTM) is a low-level programming framework for AMD's GPUs.
% computing developed by ATI/AMD.
This framework enables programmers to access AMD GPUs with a high-level abstraction, Brook+~\cite{amd-brookplus-programming},
which is an extension to the Brook GPU specification on AMD's compute abstraction layer (CAL)~\cite{amd-cal-programming}.
%, now the AMD Graphics Product Group.
%Some components of CTM and the Stream SDK are open source, such as the Brook+ C-like language and compiler,
%where Brook+ is an extension to Brook~\cite{xx}.
%, aimed at enabling GPGPU computing.
%CTM was short-lived, and the first production version of AMD's GPGPU technology is now called AMD Stream SDK,
Then AMD renamed the framework as AMD APP SDK (Accelerated Parallel Programming) built upon AMD's CAL, with an OpenCL programming interface.
%or rather the current AMD APP SDK for Windows and Linux 32-bit and 64-bit.
%APP stands for "Accelerated Parallel Processing".[1] and also targets Heterogeneous System Architecture.
In November 2015, AMD released its ``Boltzmann Initiative" and the ROCm open computing platform~\cite{rocm_url}.
% (named after Ludwig Boltzmann) in November 2015.
ROCm has a modular design which lets any hardware-vendor drivers support the ROCm stack~\cite{rocm_url}.
It also integrates multiple programming languages, e.g., OpenCL and HIP, and
provides tools for porting CUDA codes into a vendor-neutral format~\cite{hip_url}.
At the low level, ROCm is backed by a HSA-compliant language-independent runtime, which resides on the kernel driver~\cite{rocmr_url}.
%, which makes the massive body of source code written for CUDA available to AMD hardware and other hardware environments.

On AMD GPUs,
%graphics architectures,
a kernel is a single sequence of instructions that operates on a
large number of data parallel work-items. The work-items are organized into architecturally
visible work-groups that can communicate through an explicit local data share (LDS). The
shader compiler further divides work-groups into microarchitectural wavefronts that are
scheduled and executed in parallel on a given hardware implementation.
Both AMD and NVIDIA use the same idea to hide the data-loading latency and achieve high throughput,
i.e., grouping multiple threads.
AMD calls such a group a \textit{wavefront}, while NVIDIA calls it a \textit{warp}.

%It aims to provide an alternative to NVIDIA's CUDA which includes a tool to port CUDA source-code to portable (HIP)
%source-code which can be compiled on both HCC and NVCC.
%The AMD Boltzmann Initiative shall enable the porting of CUDA-based applications to a common C++ programming model.
%To summarize, there is a redical change for AMD in terms of both hardware and software.

%\begin{itemize}
%    \item Radeon Open Compute Kernel (ROCK) driver
%    \item Radeon Open Compute Runtime (ROCR) runtime
%    \item HCC: Heterogeneous Compute Compiler
%    \item HIP: C++ Heterogeneous-Compute Interface for Portability
%\end{itemize}


% COI for Intel Xeon Phis
%\subsubsection{COI for Intel Xeon Phis}
\cparagraph{MPSS/COI for Intel XeonPhis}
%Larabee~\cite{DBLP:journals/micro/SeilerCSFDJLCEGJASH09} is XXX.
Intel XeonPhi is a series of x86 manycore processors,
%for  use in supercomputers, servers, and high-end workstations.
%This architecture was
which inherit many design elements from the Larrabee project~\cite{DBLP:journals/micro/SeilerCSFDJLCEGJASH09}.
%built based on an earlier GPU design by Intel~\cite{DBLP:journals/micro/SeilerCSFDJLCEGJASH09}.
%An important component of the Intel Xeon Phi coprocessor's core is its vector processing unit (VPU),
%which features a novel 512-bit SIMD instruction set.
%To achieve its theoretical high performance,
It uses around 60 cores and 30 MB of
on-chip caches, and features a novel 512-bit vector processing unit within a core~\cite{DBLP:conf/wosp/FangSZXCV14}.
%relies on traditional many-core features
%like vector units (512-bits), high throughput, and high
%bandwidth.
%It adds to that some ``unconventional'' features, such as the overall L2 cache coherency and the ring
%interconnect, all for the sake of performance and usability.
This architecture has been used to build the Tianhe-2 supercomputer,
%which helps the National Supercomputer Center in Guangzhou
% (NSCC-GZ)
which was ranked the world's fastest supercomputer in June 2013~\cite{th2_url}.

%uses Xeon Phi processors.
%In June 2013, the Tianhe-2 supercomputer at the National Supercomputer Center in Guangzhou (NSCC-GZ) was announced[6] as the world's fastest supercomputer (as of June 2018, it is No. 4[7]). It used Intel Xeon Phi coprocessors and Ivy Bridge-EP Xeon processors to achieve 33.86 petaFLOPS.[8]

% officially known as Intel Initial Many Core Instructions (Intel IMCI).

%Since it was originally based on an earlier GPU design by Intel, it shares application areas with GPUs.[4]

The main difference between an XeonPhi and a GPU is that XeonPhi
%with an x86-compatible core,
can, with minor modifications,
run software that was originally targeted to a standard x86 CPU.
Its architecture allows the use of standard programming languages and APIs such as OpenMP.
To access the PCIe-based add-on cards,
Intel has developed the Manycore Platform Software Stack (MPSS) and the Coprocessor Offload Infrastructure (COI)~\cite{mpss_url}.
%Initially in the form of PCIe-based add-on cards, a second generation product, codenamed Knights Landing, was announced in June 2013.[5] These second generation chips could be used as a standalone CPU, rather than just as an add-in card.


Intel COI is a software library designed to ease the development of software and applications
that run on Intel XeonPhi powered device.
%The usage model is for applications that run on the host processor (e.g. Intel Xeon processor) to launch and
%communicate with workloads on one or more target devices.
The COI model exposes a pipelined programming model, which
%This model
allows workloads to be run and data to be moved asynchronously.
%, allowing the host processor,
%device processor, and DMA engines to stay busy.
%In the COI pipelining model, work flows from a "source" to a "sink".
Developers can configure one or more pipelines to interact between sources and sinks.
%Commands on these pipelines are then run in an asynchronous, in-order fashion.
%This pipelined usage model exists in a number of offload environments, including graphics and network devices,
%and has been repeatedly shown to provide a balance between high performance and programmability.
%This model can also be used as the underpinnings on other popular programming models,
%including an RPC-like environment where device work is initiated by a large number of threads on the host.
%This model is agnostic with respect to how applications and workloads are written.
COI is a C-language API that interacts with workloads through standard APIs.
%but does not impose or provide a framework for exploiting vector or thread parallelism on the host or the device.
%This allows COI to be combined with any number of other programming models, including POSIX threads,
It can be used with any other programming models, e.g., POSIX threads.
%including POSIX threads,
%Intel Parallel Building Blocks, and Intel compilers for both the host and the device.

%\cparagraph{OpenCL for Intel GPUs} Iris Graphics and Xe.

\begin{figure}[!t]
  %\includegraphics[width=0.75]{fig/ppmodel-family.pdf}
  \centering
  \includegraphics[width=0.45\textwidth]{fig/one-api.pdf}
  \caption{Intel's OneAPI software stack. Reproduced from~\cite{oneapi_url}.}
  \label{fig:one-api-sw-stack}
\end{figure}

\cparagraph{Level-Zero for Intel XPUs} Intel GPUs have been getting more powerful
and are strong contenders in the graphics and GPGPU space~\cite{DBLP:conf/cgo/ChandrasekharCC19}.
Apart from the integrated graphics, Intel has revealed its discrete GPU architecture (Xe)
targeted for datacenter and HPC applications, e.g., being as the primary compute engine for the Aurora supercomputer~\cite{aurora_url}.
%The product is intended to debut as the primary engine for
%the Department of Energy’s Aurora supercomputer in 2021.
%Accordingly, Intel has revealed its OneAPI software
Figure~\ref{fig:one-api-sw-stack} shows Intel's \texttt{OneAPI} software stack
%would be available to developers in Q4 of 2019.
%OneAPI is Intel’s effort
to unify programming across its compute product portfolio (CPUs, GPUs, NPUs and FPGAs)
with a single set of APIs~\cite{oneapi_url}.
%This facilitates a seamless transition from one XPU architecture to another.
%–its CPUs, GPUs, specialized AI silicon, and FPGAs–which the company collectively refers to as its XPUs.
%The goal of the OneAPI project is to harmonize access to those XPU technologies through a single set of APIs that makes the user feel a seamless transition from one XPU architecture to the other
At the low level, the \texttt{Level-Zero} API is to provide direct-to-metal interfaces to offload accelerator devices.
This interface is intended for providing explicit controls needed by higher-level runtime APIs and libraries, e.g., \texttt{OneAPI}.
Its design is initially influenced by other low-level APIs.
% such as OpenCL.


% DirectCompute for Win GPUs based on DirectX
%\subsubsection{DirectCompute}
\cparagraph{DirectCompute for GPUs}
Microsoft's DirectCompute is an application programming interface that supports running compute kernels
on GPGPUs
%general-purpose computing on graphics processing units
on Windows.
% Vista, Windows 7 and later versions.
DirectCompute is part of the Microsoft DirectX collection of APIs.
% and was initially released with the DirectX 11 APIs
%but runs on graphics processing units that use either DirectX 10 or DirectX 11.

DirectCompute exposes GPU's compute functionality as a new type of shader -
the compute shader, which is very similar to the existing vertex, pixel and geometry
shaders, but with much more general purpose processing capabilities~\cite{microsoft-directcompute}.
The compute shader is not attached specifically to any stage of the graphics pipeline, but
interacts with the other stages via graphics resources such as render targets, buffers and
textures. Unlike a vertex shader, or a pixel shader, the compute shader has no fixed
mapping between the data it is processing and threads that are doing the processing.
The compute shader also allows unordered memory access, in particular the ability to
perform writes to any location in a buffer.
% (also known as scattered writes).
The DirectCompute architecture shares a range of computational interfaces with NVIDIA's CUDA.
% from NVIDIA.

% Renderscript
%\subsubsection{Renderscript}
\cparagraph{Renderscript for GPUs}
Many mobile phones have followed the same
trend of desktop architectures, integrating different types of
processing units onto the same chip.
%, becoming so-called heterogeneous systems.
These new mobile phones include multi-core
CPUs (e.g., Qualcomm Snapdragon)
% NVIDIA Tegra 3,
as well as GPUs
%other special purpose processors.
% -- GPUs
%being a favorite among them --
(e.g., ARM Mali or Qualcomm Adreno).

%RenderScript is a component of the Android operating system for mobile devices that offers an API for acceleration that
%takes advantage of heterogeneous hardware. It allows developers to increase the performance of their applications
%at the cost of writing more complex (lower-level) code.
%It provides the developer three primary tools: A simple 3D rendering API, a compute API similar to CUDA, and a C99-derived language.

Google released Renderscript as an official GPU computing
framework for Android in 2011~\cite{renderscript_url}. Renderscript provides
high performance and portability across mobile hardware architectures.
%to Renderscript applications.
%Although Renderscript provides
%API for both graphics and computation, this paper focuses on
%computation.
It provides three primary tools:
a simple 3D rendering API, a compute API similar to CUDA, and a C99-derived language.

%A Renderscript application consists of three parts: (1) a host program written in Dalvik, denoted as ``.java file''
%% in Figure 1,
%(2) one or more kernels,
%and (3) reflected classes in Dalvik.
%%These three parts are denoted as 1,2, and 3 respectively in Figure 1.
%The Renderscript kernel, also written in a variant of C99,
%has a special function called root()
%that identifies the pieces of code for parallel execution.
%% in the same manner that an OpenCL kernel does.
%The  host program is similar to other Android applications but
%further initializes the use of the Renderscript kernel. The reflected
%Java classes contain functions enabling the host
%program to communicate with the kernels during runtime, allowing functions such as memory binding between
%the host program and the kernels.

%Renderscript achieves portability using LLVM [12] tech-
%nologies. Figure 1 shows the compilation flow for the Ren-
%derscript kernels. First, the Renderscript compiler “llvm-rs-
%cc”, a derivative of the Clang project, compiles Renderscript
%kernels into LLVM-based bitcode (IR) files with a .bc filename
%extension. During compilation, llvm-rs-cc also generates the
%corresponding reflected Java classes of the kernels. Thereafter,
%the bitcode is packed into an Android application package
%(.apk file) of the Renderscript application, and the application
%is installed on an Android device. When the application is
%about to execute, the bitcode is compiled to the appropriate
%machine code for the device using libbcc, the back-end com-
%piler of the Renderscript kernels.
%
%RenderScript, in turn, is a framework designed by
%Google to perform data-parallel computations in Android
%devices, transparently running user code in heterogeneous
%architectures. Differently from OpenCL, RenderScript is
%part of Android, being present in all recent versions of the
%operating system. It is a means for writing performance-critical code
%that can run effortlessly in different processors
%selected from those available at run-time, like the device's
%CPU, a DSP, or even the GPU.

%\subsubsection{Summary}
%\cparagraph{Summary}

\subsubsection{A Unified Programming Model}
%\cparagraph{the birth motivation of OpenCL}
%An industry standardization effort has recently produced the OpenCL specification for GPU programming.
%This offers the benefits of hardware-independence and reduced dependence on proprietary tool-chains.

%Graphical Processing Units (GPUs) from NVIDIA are preferentially programed with the proprietary CUDA programming toolkit.
%An alternative programming model promoted as an industry standard, OpenCL, provides similar capabilities to CUDA and
%is also supported on non-NIVIDA hardware (including multicore x86 CPUs, AMD GPUs and IBM Cell processors).

The use of heterogeneous many-core architectures in high-performance computing has attracted increasingly more interests,
particularly due to the growth of graphics processing units.
Much of this growth has been driven by NVIDIA's CUDA ecosystem for developing GPGPU applications on NVIDIA GPUs.
However, with the increasing diversity of GPUs, including those from AMD, ARM, Intel and Qualcomm,
OpenCL (Open Computing Language) has emerged as an open and vendor-agnostic standard for programming GPUs as well as other accelerating devices
%such as the APU (accelerated processing unit), FPGA (field programmable gate array), and DSP (digital signal processor).
such as APUs and FPGAs.

%OpenCL, short for Open Computing Language, is another programming environment that implements
%an accelerator programming model that is similar to CUDA. It
%Initialized by Apple Inc.,
OpenCL is an open programming standard that is maintained by the Khronos group.
%(rather than as extensions to C++ as in the CUDA API).
%As a result, OpenCL can take advantage of existing tools and compilers for a wide variety of host and GPU platforms.
%Porting OpenCL to a different host platform is a matter of providing an implementation of the runtime library that conforms
%to the standard.
%In contrast, CUDA requires a compiler that understands the extended syntax as well as an appropriate runtime library
%OpenCL was initialized by Apple Inc. and is managed
%by the Khronos Group.
%Developers can speed up application performance using OpenCL without using low-level hardware-related function calls directly.
%The OpenCL
Its API consists of a C library supporting device programming in the C99 or C++ language.
An OpenCL application is composed of two parts: one or more kernels
and an OpenCL host program.
The kernel
%, written in a restricted version of C99,
specifies functions to be executed in a parallel fashion on
the processing cores. The host sets up the execution
environment, reads in data, and instantiates and enqueues the
kernels to run.

\cparagraph{Code Portability vs. Performance Portability}\\
%To faciliate the implementation of various devices, OpenCL defines hardware abstract models for hardware-related functions.
%OpenCL is a heterogeneous computing framework that
%provides portability by defining an abstract execution model and a platform model.
OpenCL stands out in its portability by defining an abstract execution model and a platform model.
Porting OpenCL to a new many-core device is a matter of providing an implementation of
the runtime library that conforms to the standard, achieving the goal of code portability~\cite{DBLP:phd/basesearch/Fang14}.
%As a strictly defined computing standard, OpenCL has good program portability.
OpenCL applications written for one vendor's platform should run correctly on other vendors' platforms, if
they are not using any vendor-proprietary or platform-specific extensions.
The code portability of OpenCL is ensured by Khronos' certification program, which requires
OpenCL vendors to pass rigorous conformance tests on their platform before they claim it is
OpenCL ``conformant''~\cite{qualcomm_ocl_tr, opencl_cts_url}.

Different from code portability, OpenCL cannot guarantee the goal of performance portability.
This is because
%As a high-level computing standard,
the hardware implementation of OpenCL is vendor dependent.
Different hardware vendors have their unique device architectures.
% and each one may have its advantages and
%disadvantages.
As a result, an OpenCL application written and optimized for one vendor's
platform is unlikely to have the same performance as on other vendors' platforms~\cite{bodin:hal-00920910}.
To achieve portable performance, researchers have investigated various techniques,
which are discussed in Section~\ref{sec:bridge}.

%OpenCL is designed to be portable across various devices.
%However, developers must often manually adjust parameters
%such as the size of the OpenCL work-group and the hardware-dependent factors in the OpenCL application to obtain better
%performance

%Even for the same vendors, different generations of their GPU hardware may vary in micro-
%architectures and features, which could lead to noticeable performance differences for OpenCL
%programs. As a result, applications optimized for older generations of hardware often require
%fine-tuning to exploit the full capacity of newer generations.

\cparagraph{Closed and Open-source Implementation}
Table~\ref{tab:ocl-implement} shows that there exist a variety of OpenCL implementations.
%On the one hand, we notice that most vendor implementations are
%close-source, except the one from AMD and Intel.
AMD is working on the ``Boltzmann Initiative'' and the ROCm open compute platform,
which contains its OpenCL implementation~\cite{amd_opencl_url}.
Furthermore, the Gallium Compute Project
maintains an implementation of OpenCL mainly for AMD
Radeon GCN (formerly known as CLOVER~\cite{gallium_opencl_url}), and it
builds on the work of the Mesa project to support multiple
platforms.
Recently, Intel has turned to implementing OpenCL for its CPUs, GPUs and FPGAs,
and made its partial implementation open to the public~\cite{intel_opencl_url}.
BEIGNET was an open-source implementation of OpenCL released by
Intel in 2013 for its GPUs (Ivy Bridge and newer), but is now deprecated~\cite{beignet_opencl_url}.
IBM once released its OpenCL implementation for
%effective programming model for data parallel computations at
programming CEBA~\cite{DBLP:conf/ipps/BreitbartF10}.
%This open source Linux Compute project is Radeon Open Compute ROCm for
%Radeon Graphics GCN 3 and 4 (Hawaii, Fiji, Polaris) and In-
%tel Xeon E5v3 and Corev3 CPU (Haswell and newer) or new
%AMD Ryzen with PCIe Gen3 atomics capability [5].


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[!t]
\centering
\caption{The OpenCL Implementations: Open- and closed-source}
\label{tab:ocl-implement}
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{@{}llllllc@{}}
\toprule
                & Developer   & SDK            & Hardware                     & Operating System & Version  & Open-Source \\ \midrule
AMD OpenCL      & AMD         & ROCm           & AMD CPU/GPU/APU              & Linux/Windows    & 2.0      & Y           \\
\rowcolor[HTML]{C0C0C0}
NVIDIA OpenCL   & NVIDIA      & CUDA           & NVIDIA GPU                   & Linux/Windows    & 1.2      & N           \\
Intel OpenCL    & Intel       & Intel SDK      & Intel CPU/GPU/MIC/FPGA       & Linux/Windows    & 2.1      & Y           \\
\rowcolor[HTML]{C0C0C0}
IBM OpenCL      & IBM         & IBM SDK        & IBM CPU/CEBA                 & Linux            & 1.1      & N           \\
ARM OpenCL      & ARM         & ARM            & ARM CPU/Mali GPU             & Linux            & 1.2, 2.0 & N           \\
\rowcolor[HTML]{C0C0C0}
Qualcomm OpenCL & Qualcomm    & Adreno GPU SDK & Qualcomm Adreno GPU          & Andriod          & 2.0      & N           \\
TI OpenCL       & TI          & Processor SDK  & TI C66x DSP                  & Linux            & 1.1      & Y           \\
\rowcolor[HTML]{C0C0C0}
ZiiLABS OpenCL  & ZiiLABS     & ZIILABS SDK    & ZMS StemCell processors      & Andriod          & N/A      & N           \\
POCL            & Tampere U.  & POCL           & CPU/ASIP/NVIDIA GPU/HSA GPUs & Linux/Windows    & 1.2, 2.0 & Y           \\
\rowcolor[HTML]{C0C0C0}
Clover OpenCL   & Denis Steck & Mesa           & AMD GPU                      & Linux            & 1.1      & Y           \\
FreeOCL         & zuzuf       & FreeOCL        & CPU                          & Linux/Windows    & 1.2      & Y           \\
\rowcolor[HTML]{C0C0C0}
MOCL            & NUDT        & MOCL           & Matrix-2000                  & Linux            & 1.2      & Y           \\
SnuCL           & SNU         & SNUCL          & CPU/GPU/Cluster              & Linux            & 1.2      & Y           \\
\bottomrule
\end{tabular}%
}
\end{table*}

In recent years, the mobile system-on-chips (SOCs) have advanced significantly in computing
power. GPUs in the mobile SOCs are very
powerful.
To leverage the computing power, mobile vendors enable OpenCL onto their hardware.
%and some of the top mobile GPUs reach the level of console/discrete GPUs in terms of
%raw computing power.
%Despite Androidnot supporting OpenCL,
ZiiLABS enabled OpenCL on the ZiiLABS platforms and released the ZiiLABS OpenCL SDK~\cite{ziilabs_url}.
This implementation aims to unlock the full potential of the StemCell (SIMD) array architecture to
%deliver new levels of performance across a broad range of applications.
deliver new levels of performance.
%, e.g., image processing, audio processing, and graphics.
ARM has also implemented OpenCL for Mali GPUs~\cite{DBLP:conf/ipps/GrassoRRGR14}.
%we analyze performance and energy advantages of embedded GPUs for HPC. In particular, we analyze ARM Mali-T604 GPU - the first embedded GPUs with OpenCL Full Profile support. We identify, implement and evaluate software optimization techniques for efficient utilization of the ARM Mali GPU Compute Architecture. Our results show that, HPC benchmarks running on the ARM Mali-T604 GPU integrated into Exynos 5250 SoC, on average, achieve speed-up of 8.7X over a single Cortex-A15 core, while consuming only 32\% of the energy. Overall results show that embedded GPUs have performance and energy qualities that make them candidates for future HPC systems.
Qualcomm provides the Qualcomm Adreno SDK to take full advantage of
the graphics and computation power provided by the Adreno GPU~\cite{qualcomm_ocl_tr}.
To facilitate seamless migration of applications between TI SoCs,
TI has customized OpenCL implementation for its SOCs (ARM CPUs+TI DSP)~\cite{texasinstruments_ocl_url}.

%Created to tackle these problems, OpenCL allows developers to easily leverage computing power
%of mobile SOCs thanks to its cross-platform support. By using OpenCL, mobile SOCs can easily
%enable advanced use cases in many fields, such as image/video processing, computer vision,
%machine learning, etc.


%Meanwhile, the OpenCL implementation from TI is customized to
%TI SoCs (an ARM CPU + a TI DSP) [6]. On the other hand,

There are several open-source implementations developed
and maintained by the academia.
\texttt{POCL} is an implementation built on Clang and
LLVM.
%In addition to the traditional CPUs, POCL
It supports
CPUs, TTA, NVIDIA GPUs, and the HSA-based architectures~\cite{DBLP:journals/ijpp/JaaskelainenLSR15}.
%But this implementation is indeed CPU-oriented and cannot be ex-
%tended to accelerators in a straightforward way.
Based on POCL, the researchers from National University of Defense Technology have built an OpenCL implementation (\texttt{MOCL})
for the Matrix-2000 many-core architecture~\cite{DBLP:conf/cf/ZhangTFHYW18} and the FT-1500A multi-core CPU~\cite{DBLP:conf/ispa/FangZTHY17}.
With the help of the generic C++ compilers, \texttt{FreeOCL} can supports a large range of multi-core CPUs~\cite{free_opencl_url}.
\texttt{SnuCL} is an open-source OpenCL framework developed at Seoul National University.
This framework stands out that it extends the original OpenCL semantics to the heterogeneous cluster environment~\cite{DBLP:conf/ics/KimSLNJL12}.

%\cparagraph{One OpenCL to Rule them All?}
\cparagraph{One OpenCL to Rule them All?}
%For years, CUDA has been the de facto programming environment for GPGPU applications.
%In spite of this, the framework is available only on NVIDIA GPUs, traditionally requiring reimplementation
%in other frameworks to utilize additional many-core devices.
%On the other hand, OpenCL provides an open and vendor-neutral programming environment and runtime.
%With implementations available for CPUs, GPUs, and other types of accelerators,
%OpenCL therefore hods the promise of a ``write once, run anywhere'' ecosystem for heterogeneous computing~\cite{DBLP:conf/icpads/MartinezGF11}.
It has been around ten years since the birth of the OpenCL standard in 2009~\cite{ocl_url, DBLP:conf/icpads/MartinezGF11}.
%At the very beginning,
We had expected that, OpenCL became the unified de facto standard programming model for heterogeneous many-core processors,
like OpenMP for multi-core CPUs~\cite{omp_url} and MPI for large-scale clusters~\cite{mpi_url}.
However, this is not the case.
% up to now.
The fact is that, CUDA has been the de facto programming environment on GPGPUs for years.
Table~\ref{tab:sc-top10-ppm} shows that five of the top ten supercomputers
use GPGPU architectures and take CUDA as their programming methodology.

We believe that there are several factors behind OpenCL's tepid popularity.
The first factor is due to the diversity of many-core architectures in terms of processing cores and memory hierarchies.
For example, using scratch-pad memory has been very popular in DSPs, game consoles (IBM Cell/B.E.), and graphic processor,
while caches are typically used in Intel XeonPhi.
To be compatible with the diverse many-cores, the next version of the OpenCL standard will
let more OpenCL features become optional for enhanced deployment flexibility.
The optionality includes both API and language features e.g., floating point precisions.
By doing so, we can enable vendors to ship functionality precisely targeting their customers and markets~\cite{opencl-architecture-update-whitepaper}.
The second factor is due to the commercial interests.
The vendors would prefer using a specialized programming model for their hardware and building a complete software ecosystem.
From the perspective of programmers, we often choose to use the CUDA programming interface for NVIDIA GPU.
This is because NVIDIA optimize its CUDA software stack, and
thus applications in CUDA can often enable us to yield a better performance~\cite{DBLP:conf/icpp/FangVS11}.

%(1) commercial interests, (2) the diversity of many-core architectures, and (3) many others.

%CUDA is still the main programming approach on NVIDIA GPUs.
%For years, CUDA has been the de facto programming environment for GPGPU applications.
%Table~\ref{tab:sc-top10-ppm} shows that five of the top ten supercomputers uses CPU-GPUs architectures, which leverage CUDA as their programming methodology.
%HIP is the one on AMD GPUs, although AMD still supports OpenCL for its hardware.
%Intel has released its OneAPI stategy, while it still supports OpenCL for its FPGAs and GPUs.

%To summarize,
To summarize, \textit{OpenCL is eligible, yet not practical to be a unified programming model for heterogeneous many-core architectures}.
For future, we argue that, neither OpenCL nor CUDA dominates the programming range for heterogeneous many-core architectures,
but it is likely that they coexist.
Our investigation work shows that the low-level programming models share a common working paradigm,
and vendors would choose to support their unique one.
%, vendors choose to support different low-level programming models.
%The important thing is that vendors have implementations of one or more native programming models and build a complete ecosystem around it.
Thereafter, they should develop a complete ecosystem (e.g., domain libraries) around this programming model.


==> pp-models - Copy/lst/source_in.tex <==
//setting the partition-size and task granularity
hStreams_app_init(partition_size,streams_p_part);

//stream queue id
stream_id = 0;
for(...){
  //enquque host-device transfer to current stream
  hStreams_app_xfer_memory(,,, stream_id, HSTR_SRC_TO_SINK,...);
  ...
  //enqueue computation to the current stream
  hStreams_EnqueueCompute(stream_id, "kernel1", ...);
  ...
  //move to the next stream
  stream_id = (stream_id++) % MAX_STR;
}
//transfer data back to host
hStreams_app_xfer_memory(,,, HSTR_SINK_TO_SRC,...);


==> pp-models - Copy/lst/source_out.tex <==
__kernel void A(__global char* a, short b, int c) {
  const int d = get_global_id(0);
  a[d] = b;
}

==> pp-models - Copy/next.tex <==
\section{A Vision for the Next Decade} \label{sec:next}
Given the massive performance potential of heterogeneous many-core hardware design, it is clear that future computing hardware will be
increasingly specialized and diverse. As the hardware design keeps evolving, so does the software development systems and the programming
model. In this section, we discuss some challenges and open research directions for future parallel programming models.

%\vspace{-2mm}
\cparagraph{A holistic solution.} China, US, Japan and EUROPE are currently working towards the exascale computing.
%The next major milestone in supercomputing is
The design and construction of an exascale machine will be built based on
%and the
heterogeneous many-core architectures of various forms~\cite{DBLP:journals/jzusc/LiaoLYLYLHLFRS18}.
%Nonetheless, introducing a much larger number of compute nodes
%meeting memory bandwidth and power consumption requirements,
%as well as the wide-scale scientific deployment of heterogeneous architectures,
%will not lead to a sustanable exascale computing system.
%Rather,
This achievement will require significant advances in the software paradigm
%governing the production of scientific program codes
and require that parallelism in control and data be exploited at all possible levels.
Therefore,
%Currently, China, US, Japan and EUROP are working close to reach the exascale.
%We argue that the hardware architectures will be more diverse and in a heterogeneous form.
the dominant design parameter
%governing performance
will shift from hardware to system software and
in particular, parallel programming systems~\cite{DBLP:journals/tjs/DavisRFNT12}.
We envision that a hierarchy of programming models have to be implemented as well as the equipment of expert optimized libraries.
Low-level programming models should be implemented, but are not suggested to be exposed to programmers.
Instead, the high-level programming models and highly optimized domain libraries are exposed as the programming interface.
Intel's OneAPI is one of such examples~\cite{oneapi_url}.
%We have little belief in the one-size-fits-all for sci-entific computing.

%\vspace{-2mm}
\cparagraph{Pattern-aware parallel programming.} Parallel programming based on patterns (such as \textit{map/reduce} and \textit{pipeline})
or algorithmic skeletons (Section \ref{sec:skeleton}), where programmers write algorithmic intents that abstract away parallelization,
heterogeneity, and reliability concerns, offer a partial solution for programming heterogeneous parallel systems~\cite{de2017bringing}. As
can been from Section~\ref{sec:highlevel-ppm}, this is an essential feature of high-level parallel programming models. The key to the
success of pattern-based parallel programming is to have a fully-supported development toolchain for code optimization, debugging and
performance diagnosis. The current compiler implementation is oblivious to the high-level algorithmic intents expressed in the patterns,
leading to disappointing performance, discouraging the adoption of pattern-based parallel programming. For example, a sequential loop that
adds one to an integer literal one million times will be optimized away at compile time. However, if we implement it as a parallel pipeline
pattern, existing compilers, including leading industrial parallel compilers, Intel TBB on ICC and Go, would fail to merge the trivial
pipeline elements. As a result, the pattern-based implementation takes minutes to run, not nanoseconds\footnote{Code is available at:
\url{https://goo.gl/y7bBdN}.}, leading to a massive slowdown over the sequential version. The issue arises from the fact that current
compilers are oblivious to parallel patterns. A parallel construct encodes the sequential semantics of the program, but this is lost to the
compiler. If the compiler knew the sequential semantics, it can then dynamically merge small pipeline elements. If we can do these, the
primary barrier to adopting pattern-based programming would be torn down.


%\vspace{-2mm} \cparagraph{Open standard is important.} We should not overlook the legacy scientific software that has existed for decades.
%While it often infeasible to re-implement legacy code to port them to new programming model, many of the legacy sciatica applications
%require high-performance.
%%This has the drawback captured in Amdahl's law, where the serial part of the code quicklybecomes the bottleneck.
%Therefore, vendors should continue supporting the open programming standard such as OpenCL or SYCL, to be compatible with the legacy codes.


%\vspace{-2mm}
\cparagraph{Machine learning based program tuning.} Programmers are faced with many decisions when writing heterogeneous programs, such as
selecting an optimal thread configuration~\cite{DBLP:journals/tpds/DaoL18} and/or selecting a right code
variant~\cite{DBLP:conf/asplos/MuralidharanRHG16}. This is due to the profound differences in many-core architectures, programming models
and input applications~\cite{DBLP:journals/pieee/BalaprakashDGHH18}. By default, the runtime system of high-level programming models has to
assist users in automating these online decisions. If a wrong configuration is selected, the overall performance will be significantly
decreased. Therefore, it is significant to design a model to help programmers to automatically choose a reasonable configuration, i.e.,
\textit{automated performance tuning}, which is regarded to have the potential to dramatically improve the performance portability of
petascale and exascale applications~\cite{DBLP:journals/pieee/BalaprakashDGHH18}. A key enabling technology for optimizing parallel
programs is \emph{machine learning}. Rather than hand-craft a set of optimization heuristics based on compiler expert insight, learning
techniques automatically determine how to apply optimizations based on statistical modelling and learning~\cite{zhengphd,mlcpieee}. This
provides a rigorous methodology to search and extract structure that can be transferred and reused in unseen settings.  Its great advantage
is that it can adapt to changing platforms as it has no a priori assumption about their behaviour. There are many studies showing it
outperforms human-based approaches. Recent work shows that it is effective in performing parallel code
optimization~\cite{grewe2013portable,DBLP:journals/taco/WangGO14,cc14,ogilvie2014fast,cgo17,cummins2017end,chen2020characterizing},
performance predicting~\cite{zhao2016predicting,wang2013using}, parallelism
mapping~\cite{Tournavitis:2009:THA:1542476.1542496,wang2010partitioning,grewe2013opencl,DBLP:journals/taco/WangGO14,wen2014smart,wang2014integrating,taylor2017adaptive,tpds20},
and task scheduling~\cite{emani2013smart,ren2017optimise,conext18,yuan2019using,ren2020camel,sanz2019optimizing}. As the many-core design
becomes increasingly diverse, we believe that the machine-learning techniques provide a rigorous, automatic way for constructing
optimization heuristics, which is more scalable and sustainable, compared to manually-crafted solutions.


==> pp-models - Copy/overview.tex <==
\section{Overview of Parallel Programming Models} \label{sec:overview}
\begin{figure}[!b]
	%\includegraphics[width=0.75]{fig/ppmodel-family.pdf}
	%\centering
	\includegraphics[width=0.52\textwidth]{fig/ppmodel-family.pdf}
	\caption{The family of parallel programming models for heterogeneous many-core architectures.}
	\label{fig:ppmodel-family}
\end{figure}
Parallel programming model acts as the bridge between programmers and
%heterogeneous many-core architectures.
parallel architectures.
%For the exploitation of 
To use the shared memory parallelism on multi-core CPUs, 
parallel programming models are often implemented on threading mechanisms such as the POSIX threads~\cite{DBLP:conf/usenix/Alfieri94}.
When it comes to heterogeneous many-cores, we have to deal with the heterogeneity between host and accelerators.
%Accordingly, 
And parallel programming models have to introduce relevant abstractions of controlling them both,
%both host and accelerators, 
which is the focus of this survey work. 
%In this work, we focus on reviewing programming models for heterogeneous many-cores. 

%parallel processors.
%In this work, we focus on the programming models for heterogeneous many-core architectures.
Figure~\ref{fig:ppmodel-family} summarizes
the family of parallel programming models for heterogeneous many-core architectures.
Based on the performance-programmability tradeoff,
% of performance and programmability, 
%we categorize parallel programming models into
we categorize them into
\textit{low-level programming models} (Section~\ref{sec:lowlevel-ppm}) and \textit{high-level programming models} (Section~\ref{sec:highlevel-ppm}).
%, and \textit{domain-specific programming models}.
%Overall, the 
The expected application \textit{performance} increases from high-level programming models to low-level programming models, 
whereas the \textit{programmability} decreases.
%accordingly.


The low-level programming models are closest to the many-core architectures, and
expose the most hardware details to programmers through data structures and/or APIs.
These models are typically bound to specific hardware architectures, and are also
%Thus, the low-level programming models are also
known as \textit{native programming models}.
In contrast, the high-level programming models raise the languages' abstraction level,
%based on the low-level programming models,
%and can be mapped to more heterogeneous architectures than the low-level models.
and hide more architecture details than the low-level models. 
Thus, the high-level models often enable better programmability.

%The domain-specific programming models further raise the language's abstraction level with
%domain-speciﬁc data types, operators, and control constructs,
%thus enabling the best programmability.


==> pp-models - Copy/preamble.tex <==
\usepackage{booktabs}
\usepackage{graphicx}
\usepackage{lscape}
\usepackage[table,xcdraw]{xcolor}
\usepackage{listings}
\usepackage{cite}
\usepackage[tight,footnotesize]{subfigure}
\usepackage{xspace}
%\usepackage[misc,geometry]{ifsym}
\usepackage{marvosym}
\usepackage{balance}
\usepackage{url}

\newcommand\etal{\emph{et al.}\xspace}
\newcommand\cparagraph[1]{\vspace{1.5mm}\noindent \textbf{#1}}
%\newcommand\cparagraph[1]{\vspace{1.0mm}\noindent \textbf{#1}}
\newcommand\FIXME[1]{\textcolor{red}{FIX:}\textcolor{red}{#1}}

\definecolor{mygreen}{rgb}{0,0.6,0}
\lstset{%
  basicstyle=\scriptsize,%
  numbers=left,%
  xleftmargin=2em,
  framexleftmargin=2em,
  escapeinside={@|}{|@},
  frame=b,%
  breaklines=true,%
  commentstyle=\color{mygreen},
  postbreak=\raisebox{0ex}[0ex][0ex]{\ensuremath{\color{red}\hookrightarrow\space}},%
  % red arrow at line breaks
  captionpos=b%,
  keywordstyle=\color{blue},       % keyword style
  language=C,
  morekeywords={*,stream_id,partition_size,streams_p_part,hStreams_app_init},           % if you want to add more keywords to the set
  stepnumber=2,
}


==> pp-models - Copy/stream.tex <==
%\section{The Streaming Mechanism in Programming Models}
%\section{ Host-Accelerator Communication Optimization Techniques} \label{sec:stream}
\section{Optimization Techniques for Minimizing the Host-Accelerator Communication} \label{sec:stream}
While the heterogeneous many-core design offers the
potential for energy-efficient, high-performance computing,
software developers are finding it increasingly hard to deal
with the complexity of these systems~\cite{DBLP:journals/ijhpca/MeswaniCUSBP13, DBLP:conf/icpp/FangVS11}.
In particular, programmers need to effectively manage the host-device
communication, because the communication overhead can
completely eclipse the benefit of computation offloading
if not careful~\cite{DBLP:conf/ispass/GreggH11, DBLP:conf/iiswc/CheBMTSLS09, DBLP:conf/ipps/BoyerMK13, DBLP:conf/wosp/FangSZXCV14}.
Gregg and Hazelwood have
shown that, when memory transfer times are included,
it can take 2x--50x longer to run a kernel than the GPU processing time alone~\cite{DBLP:conf/ispass/GreggH11}.

%To this end, heterogeneous streaming has been proposed as a solution
Various parallel programming models have introduced the streaming mechanism to
amortize the host-device communication cost~\cite{DBLP:conf/ipps/NewburnBWCPDSBL16}.
It works by partitioning the processor
cores to allow independent communication and computation
tasks (i.e., streams) to run concurrently on different hardware
resources, which effectively overlaps the kernel execution
with data movements.
Representative heterogeneous streaming implementations include CUDA Streams~\cite{cuda_url}, OpenCL
Command Queues~\cite{ocl_url}, and Intel's hStreams~\cite{tr:hstreams:arch, DBLP:conf/ipps/NewburnBWCPDSBL16, DBLP:conf/npc/LiFTCY16, DBLP:journals/ppl/FangZLTCCY16, DBLP:conf/ipps/ZhangFTYW18, DBLP:conf/ipps/LiFTCCY16}.
These implementations allow the program to spawn more
than one stream/pipeline so that the data movement stage of
one pipeline overlaps the kernel execution stage of another.


%\vspace{-1mm}
\subsection{The Streaming Mechanism}
The idea of heterogeneous streams is to exploit temporal and spatial sharing of the computing resources.

\begin{figure}[!t]
\centering
\includegraphics[width=0.45\textwidth]{./dia/temporal_sharing.pdf}
\caption{Exploit pipeline parallelism by temporal sharing. Reproduced from \cite{DBLP:conf/ipps/ZhangFTYW18}.}
\label{fig:temporal_sharing}
\end{figure}

\cparagraph{Temporal Sharing.} Code written for heterogeneous computing devices typically consists of several stages such as host-device
communication and computation. Using temporal sharing, one can overlap some of these stages to exploit pipeline parallelism to improve
performance. This paradigm is illustrated in Figure~\ref{fig:temporal_sharing}. In this example, we can exploit temporal sharing to overlap
the host-device communication and computation stages to achieve better runtime when compared to  execute every stage sequentially.
%One way of exploiting temporal sharing is to group fine-grained independent tasks into groups so that each group can
%run in a pipeline fashion.
One way of exploiting temporal sharing is to divide an application into independent tasks so that they can run in a pipeline fashion.


Note that the PPE and SPEs of Cell/B.E. share the same memory space, and
thus there is no need of host-accelerator communication~\cite{DBLP:journals/ibmrd/ChenRDI07}.
But each SPE has a channel/DMA transport for controlling input and output.
To prevent memory stalls, we can take advantage of the DMA engines by
adopting a double-buffer approach to overlap computations on the previously fetched datablocks
with transfers of subsequent data blocks to and from memory.
We regard that this is a special case of \textit{temporal sharing}.

\cparagraph{Spatial Sharing.}
Using multiple streams also enjoys the idea of resource partitioning. That is, to partition the resource (e.g., processing cores) into multiple groups and map each stream onto a partition. Therefore, different streams can run on different partitions concurrently, i.e., resource \textit{spatial sharing}. Nowadays accelerators have a large number of processing units that some applications cannot efficiently exploit them for a given task. Typically, we offload a task and let it occupy all the processing cores. When using multiple streams, we divide the processing cores into multiple groups (each group is named as a \textit{partition}). Figure~\ref{fig:spatial_sharing} shows that a device has 16 cores and is logically divided into four partitions (\texttt{P0}, \texttt{P1}, \texttt{P2}, \texttt{P3}). Then different tasks are offloaded onto different partitions, e.g., \texttt{T0}, \texttt{T1}, \texttt{T2}, \texttt{T3} runs on \texttt{P0}, \texttt{P1}, \texttt{P2}, \texttt{P3}, respectively. In this way, we aim to improve the device utilization.

\begin{figure}[!t]
\centering
\includegraphics[width=0.45\textwidth]{./dia/spatial_sharing.eps}
\caption{Spatial sharing. The circles represent processing cores, \texttt{Tx} represents a task, and \texttt{Px} represents a partition. }
\label{fig:spatial_sharing}
\end{figure}

\vspace{-4mm}
\subsection{Intel hStreams}
Intel \texttt{hStreams} is an open-source streaming implementation built on the COI programming model~\cite{DBLP:conf/ipps/NewburnBWCPDSBL16}.
At its core is the resource partitioning mechanism~\cite{tr:hstreams:arch}.
%Figure~\ref{fig:hstreams_resource_view} shows the mapping between logical concepts and a physical machine (e.g., Intel Xeon Phi).
At the physical level, the whole device is partitioned into multiple groups and thus each group has several processing cores. At the logical level, a device can be seen as one or more \textit{domains}. Each domain contains multiple \textit{places}, each of which then has multiples \textit{streams}. The logical concepts are visible to programmers, while the physical ones are transparent to them and the mapping between them are automatically handled by the runtime.

\texttt{hStreams} is implemented as a library and provides users with APIs to access coprocessors/accelerators efficiently.
Programming with \texttt{hStreams} resembles that in \texttt{CUDA} or \texttt{OpenCL}.
Programmers have to create the streaming context, move data between host and device, and invoke kernel execution.
And they also have to split tasks to use multiple streams.
%Further, \texttt{hStreams} cannot be used alone, but has to used with other programming models such as \texttt{OpenMP} or Intel \texttt{TBB}.
Figure~\ref{fig:example_code} gives a simplified code example written with Intel's \texttt{hStreams} APIs.
At line 2, we initialize the stream execution by setting the number of partitions and tasks/streams per partition.
This initialization process essentially creates multiple processor domains and
determines how many logical streams can run on a partition.
In the \emph{for} loop (lines 7-14) we enqueue the communication and computation tasks to a number of streams identified by the
\texttt{stream\_id} variable. In this way, communication and computation of different streams can be overlapped during execution
(temporal sharing); and streams on different processor domains (or partitions) can run concurrently (spatial sharing).
%Our predictive model determines the \textit{\#partitions} and the \textit{\#tasks} before invoking the \texttt{hStreams} initialization routine,
%\texttt{hStreams\_app\_init()}. We also create a wrap for this API to automatically invoke our predictive model, so no modification to the
%application source code is required.

\lstset{}
\begin{figure}[!t]
	\centering %
		\noindent\mbox{\parbox{\columnwidth}{%
				\lstinputlisting[label=subfig:source_in]{lst/source_in}%
		}}
    \vspace{-3mm}
	\caption{Example \texttt{hStreams} code.}%
	\label{fig:example_code}%
\end{figure}
%\subsection{Selecting an Optimal Stream Configuration}
\subsection{Performance Modelling for Streaming Programs}
% motivation
%Consider Figure~\ref {fig_motivation_overall} which shows the resultant performance improvement over the non-streamed version of the code
%for two applications on a 57-core Intel XeonPhi system. It is observed from this example that no all stream configurations give  improved
%performance. As can be seen from the diagrams, the search space of stream configuration is huge but good configurations are sparse. The
%performance varies significantly over stream configurations (\textit{\#partitions}, \textit{\#tasks}). The optimal \textit{\#tasks} for
%\texttt{binomial} ranges from 1 to 30, and the best \textit{\#partitions} is between  1 and 40. In contrast to \texttt{binomial},
%\texttt{prefixsum} benefits from fine-grained parallelism when using a larger \textit{\#tasks} (220 to 224) and \textit{\#partitions} (60
%to 80). However, the stream configurations that are effective for \texttt{prefixsum} give no speedup over the non-streamed version for
%\texttt{binomial}.

%\begin{figure*}[!t]
%\centering
%\subfigure[\texttt{binomial}]{\label{fig_motivation_partition_cf}\includegraphics[width=0.48\textwidth]{data/binomial_16384.pdf}}
%\subfigure[\texttt{prefixsum}]{\label{fig_motivation_partition_mm}\includegraphics[width=0.48\textwidth]{data/prefixsum-n26.pdf}}
%\caption{Heatmaps show the resultant speedup (over non-streamed) of \texttt{binomial} and \texttt{prefixsum} under different
%stream configurations. The \textit{\#partitions} and \textit{\#tasks}  have a significant impact on the resultant performance, and the sweat spots vary across programs. Reproduced from \cite{DBLP:conf/ipps/ZhangFTYW18}.}
%\label{fig_motivation_overall}
%\end{figure*}

%These two examples
The previous work have demonstrated that choosing a right stream configuration
has a great impact on the resultant performance~\cite{DBLP:conf/ipps/ZhangFTYW18, DBLP:journals/ppl/FangZLTCCY16}.
And the best configuration must be determined on a per-program and per-dataset basis.
Attempting to find the optimal configuration through
%means of
an exhaustive search would be ineffective,
and the overhead involved would be far bigger than the potential
benefits. Therefore, building models for heterogeneous streaming programs is of great significance.
%Online search algorithms, while can speedup the search process, the overhead can still outweigh the benefit. For example, when
%applying simulated annealing to \texttt{binomial}, the best-found configuration only reaches 84\% of the best-available performance after
%310,728 iterations\footnote{Later in Section~\ref{sec:overall}, we show that our approach achieves 98\% of the best-available performance
%for \texttt{dct}.}.

%One the one hand,
% \cparagraph{Classical hand-written heuristics.}
\subsubsection{Hand-Crafted Analytical Models}
\vspace{-2mm}
% are not ideal either, as they are not only complex to develop, but are likely to fail
%due to the variety of programs and the ever-changing hardware architecture.
%In,
Gomez-Luna \etal present performance models for asynchronous data transfers on
 GPU architectures~\cite{DBLP:journals/jpdc/Gomez-LunaGBG12}.
The models permit programmers to estimate the optimal number of streams in which the computation on the GPU should be broken up.
%In~\cite{DBLP:conf/ccgrid/WerkhovenMSB14},
Werkhoven \etal present an analytical performance model to indicate when to
apply which overlapping method on GPUs~\cite{DBLP:conf/ccgrid/WerkhovenMSB14}.
The evaluation results show that the performance model is capable of correctly classifying the relative performance of the different implementations.
%In~\cite{DBLP:journals/ijhpca/LiuQJG16},
Liu \etal carry out a systematic investigation into task partitioning to
achieve maximum performance gain for AMD and NVIDIA GPUs~\cite{DBLP:journals/ijhpca/LiuQJG16}.
%Unlike these works, we discuss the heuristics of reducing the search space when determining the factors. Using a model on Phi will be investigated as our future work.
This approach is not ideal, as it is not only complex to develop the analytical models, but is likely to fail
due to the variety of programs and the ever-changing hardware architecture.
That is, these hand-crafted models have the drawback of being not
portable across architectures as the model is tightly coupled to a specific many-core architecture.

%\cparagraph{Multiple Streams Modeling.}
%Gomez-Luna \etal~\cite{citeulike:9715521} develop a set of models to estimate the asynchronous data
%transfer overhead on different GPU architectures.
%The models can be used to estimate the optimal number of streams to use on a given GPU
%platform. Werkhoven \etal~\cite{citeulike:13920334} present an analytical model to determine  when to apply an overlapping method on GPUs.
%Liu \etal~\cite{citeulike:13920353} also develop an analytical based approach to determine the optimal number of streams to use on GPUs.
%However, none of these approaches considers the processor partition. As we have shown in Section~\ref{sec:alt}, ignoring the processor
%partitioning parameter can lead to poor performance on Intel XeonPhi. Furthermore, these hand-crafted models have the drawback of being not
%portable across architectures as the model is tightly coupled to a specific GPU architecture.
%Our work advances prior work by employing
%machine learning to automatically learn the optimal processor partition and the number of streams/tasks to use. Since our models are
%automatically learned from empirical observations, one can easily re-learn a model for a new architecture.


%One the other hand,
%An alternate approach, and the one we chose to use, is to use
%\cparagraph{Models built on machine-learning techniques.}
\subsubsection{Machine-Learning based Models}
\vspace{-2mm}
Researchers have also exploited the machine learning techniques to automatically construct a predictive model to
directly predict the best configuration~\cite{DBLP:conf/ipps/ZhangFTYW18, tpds20}.
This approach provides minimal runtime, and
has little development overhead when targeting a new many-core architecture.
%This paper presents a novel runtime approach to determine the right number of partitions and tasks for heterogeneous streams, targeting the
%Intel XeonPhi architecture.
This is achieved by employing machine learning techniques to automatically construct a predictive model to decide at
runtime the optimal stream configuration for
any streamed application.
The predictor is first trained \emph{off-line}. Then, using code and dynamic runtime features of the program,
the model predicts the best configuration for a \emph{new}, \emph{unseen} program.
This approach can avoid the pitfalls of using a hard-wired
heuristic that requires human modification every time when the architecture evolves,
where the number and the type of cores are likely to change from one generation to the next.
Experimental results XeonPhi and GPGPUs have shown that this approach can achieve over 93\% of the Oracle performance~\cite{tpds20}.

